Web Question Answering with Neurosymbolic Program Synthesis

In this paper, we propose a new technique based on program synthesis for extracting information from webpages. Given a natural language query and a few labeled webpages, our method synthesizes a program that can be used to extract similar types of information from other unlabeled webpages. To handle websites with diverse structure, our approach employs a neurosymbolic DSL that incorporates both neural NLP models as well as standard language constructs for tree navigation and string manipulation. We also propose an optimal synthesis algorithm that generates all DSL programs that achieve optimal F1 score on the training examples. Our synthesis technique is compositional, prunes the search space by exploiting a monotonicity property of the DSL, and uses transductive learning to select programs with good generalization power. We have implemented these ideas in a new tool called WebQA and evaluate it on 25 different tasks across multiple domains. Our experiments show that WebQA significantly outperforms existing tools such as state-of-the-art question answering models and wrapper induction systems.

==> WebExtract arxiv/ablation-ex.tex <==
    \definecolor{warmgrey}{RGB}{121,125,98}
    \definecolor{coolgray}{RGB}{38,70,83}
    \definecolor{deeporange}{RGB}{244,162,97}
    \definecolor{cadmiumorange}{RGB}{231,111,81}
    \definecolor{greyolive}{RGB}{155,155,122}
    \definecolor{peachbeige}{RGB}{217,174,72}
    \definecolor{yellowbeige}{RGB}{241,220,167}
    \definecolor{yellowochre}{RGB}{255,203,105}
    \definecolor{nectar}{RGB}{208,140,96}
    \begin{tikzpicture}[scale=0.9]
        \begin{axis}[
            ylabel near ticks,
            ymax= 1.0,
            % xmax=1,
            % legend cell align = left,
            % legend pos =  north east,
            legend style = {nodes={scale=0.8, transform shape}, anchor=north, at={(0.5, 1.12)}, legend columns=4, draw=none},
            xlabel style={yshift=1mm},
            ylabel = $F_1$ score,
            xlabel = \# of examples,
            % x dir=reverse
        ]
        \legend{${\tt conf}_{t1}$, ${\tt conf}_{t2}$, ${\tt conf}_{t3}$, ${\tt conf}_{t4}$, ${\tt conf}_{t5}$, ${\tt conf}_{t6}$}
        \addplot[
            % smooth,
            line width=0.3mm,
            mark=square*,
            color=warmgrey
        ] coordinates {
            (5, 0.659)
            (4, 0.611)
            (3, 0.562)
            (2, 0.577)
            (1, 0.095)
        };
        \addplot[
            % smooth,
            line width=0.3mm,
            mark=*,
            color=coolgray
        ] plot coordinates {
            (5, 0.740)
            (4, 0.740)
            (3, 0.740)
            (2, 0.740)
            (1, 0.251)
        };

        \addplot[
            % smooth,
            line width=0.3mm,
            mark=triangle*,
            color=peachbeige
        ] plot coordinates {
            (5, 0.638)
            (4, 0.527)
            (3, 0.568)
            (2, 0.568)
            (1, 0.134)
        };
        
        \addplot[
            % smooth,
            line width=0.3mm,
            mark=diamond,
            color=cadmiumorange
        ] plot coordinates {
            (5, 0.500)
            (4, 0.314)
            (3, 0.325)
            (2, 0.240)
            (1, 0.211)
        };
        \addplot[
            % smooth,
            line width=0.3mm,
            mark=x,
            color=yellowochre
        ] plot coordinates {
            (5, 0.913)
            (4, 0.913)
            (3, 0.851)
            (2, 0.800)
            (1, 0.800)
        };
        \addplot[
            % smooth,
            line width=0.3mm,
            mark=o,
            color=nectar
        ] plot coordinates {
            (5, 0.727)
            (4, 0.727)
            (3, 0.713)
            (2, 0.696)
            (1, 0.489)
        };
        \end{axis}
    \end{tikzpicture}
    
    % \captionsetup{font={footnotesize}}
    %\caption{Number of benchmarks solved over iterations for StackOverflow data set.}\label{fig:so-solved}


==> WebExtract arxiv/ablation-input.tex <==
    \definecolor{coolgray}{RGB}{38,70,83}
    \definecolor{powderblue}{RGB}{190,227,219}
    \definecolor{peachbeige}{RGB}{255,214,186}
    \definecolor{champagnepink}{RGB}{237,221,212}
\begin{tikzpicture}[scale=0.9]
\begin{axis}[
    ymin=0,
    ymax=0.8,
    ybar,
    enlarge x limits=0.20,
    legend style={at={(0.5,-0.15)},
      anchor=north,legend columns=-1},
    ylabel={Avg $F_1$},
    symbolic x coords={Faculty,Conference,Class, Clinic},
    xtick=data,
    legend image code/.code={
        \draw [#1] (0cm,-0.1cm) rectangle (0.2cm,0.25cm); },
    ]
\addplot[black,fill=champagnepink
] coordinates {(Faculty, 0.22) (Conference, 0.42) (Class, 0.35) (Clinic, 0.49)};
\addplot[black,fill=coolgray
] coordinates {(Faculty, 0.68) (Conference, 0.57) (Class, 0.52) (Clinic, 0.647)};
\addplot[black,fill=powderblue
] coordinates {(Faculty, 0.74) (Conference, 0.70) (Class, 0.69) (Clinic, 0.657)};
\legend{\toolname-{\sc NL},\toolname-{\sc KW},\toolname}
\end{axis}
\end{tikzpicture}

==> WebExtract arxiv/abstract.tex <==
\begin{abstract}
In this paper, we propose a new technique based on program synthesis for extracting information from webpages. Given a natural language query and a few labeled webpages, our method synthesizes a program that can be used to extract similar types of information from other unlabeled webpages. To handle websites with diverse structure, our approach employs a neurosymbolic DSL that incorporates both neural NLP models as well as standard language constructs for tree navigation and string manipulation. We also propose an optimal synthesis algorithm that generates all DSL programs that achieve optimal $F_1$ score on the training examples. Our synthesis technique is compositional, prunes the search space by exploiting a  monotonicity property of the DSL, and uses transductive learning to select programs with good generalization power. We have implemented these ideas in a new tool called \toolname and evaluate  it on 25 different tasks across multiple domains. Our experiments show that \toolname significantly outperforms existing tools such as state-of-the-art question answering models and wrapper induction systems. 
\end{abstract}



==> WebExtract arxiv/baselinecomp2.tex <==
\definecolor{independence}{RGB}{121,125,98}
\definecolor{heliotropegray}{RGB}{154,140,152}
\definecolor{silverpink}{RGB}{201,173,167}
\definecolor{isabelline}{RGB}{242,233,228}

\definecolor{usafablue}{RGB}{0,78,137}
\definecolor{orangecrayola}{RGB}{255,107,53}
\definecolor{peachcrayola}{RGB}{247,197,159}
\definecolor{beige}{RGB}{239, 239, 208}

\definecolor{darkbluegray}{RGB}{102,106,134}
\definecolor{shadowblue}{RGB}{120,138,163}
\definecolor{opal}{RGB}{146,182,177}
\definecolor{laurelgreen}{RGB}{178,201,171}
\definecolor{dutchwhite}{RGB}{232,221,181}
\begin{tikzpicture}[scale=0.9]
\begin{axis}[
    ymin=0,
    ymax=0.8,
    ybar,
    enlarge x limits=0.20,
    legend style={at={(0.5,-0.15)},
      anchor=north,legend columns=-1},
    ylabel={Avg score},
    symbolic x coords={$F_1$,Precision,Recall},
    xtick=data,
    % nodes near coords,
    % nodes near coords, align={vertical}
    legend image code/.code={
        \draw [#1] (0cm,-0.1cm) rectangle (0.2cm,0.25cm); },
    ]
\addplot[black,fill=darkbluegray
% postaction={pattern=horizontal lines}
] coordinates {($F_1$, 0.70) (Precision, 0.69) (Recall, 0.73)};
\addplot[black,fill=opal
% postaction={pattern=vertical lines}
] coordinates {($F_1$, 0.25) (Precision, 0.47) (Recall, 0.17)};
\addplot[black,fill=peachcrayola
% postaction={pattern=north east lines}
] coordinates {($F_1$, 0.05) (Precision, 0.34) (Recall, 0.03)};
\addplot[black,fill=dutchwhite
% postaction={pattern=north west lines}
] coordinates {($F_1$, 0.08) (Precision, 0.06) (Recall, 0.15)};
\legend{\toolname,{\sc BERTQA},{
    \sc HYB}, {\sc EntExtract}}
\end{axis}
\end{tikzpicture}

==> WebExtract arxiv/concl.tex <==
\section{Conclusion}\label{sec:concl}

We have presented \toolname, a new synthesis-powered system for extracting information  from webpages. 
%Given a few labeled webpages, \toolname synthesizes programs that achieve maximum $F_1$ score on the provided examples. To handle a diverse set of structurally heterogeneous websites, \toolname synthesizes programs in a neurosymbolic DSL that combines tree navigation and string manipulation constructs with neural NLP modules for question answering, keyword matching, and entity extraction. However, since the synthesis problem has \emph{many} optimal solutions, \toolname also uses a new (ensemble-based) self-supervised learning technique to choose a program with good generalization power. 
We have evaluated \toolname on 25 different tasks spanning four different domains and 160 different webpages and show that \toolname significantly outperforms competing approaches in terms of $F_1$ score, precision, and recall. 


==> WebExtract arxiv/dsl.tex <==
\section{DSL for Web Question Answering}\label{sec:dsl}

In this section, we describe our domain-specific language called \dsl for web information extraction. At a high level, this DSL  combines pre-trained neural models for standard NLP tasks (i.e., question answering, entity extraction, and keyword matching) with symbolic constructs for manipulating strings and navigating the tree structure of the webpage. As shown in Figure~\ref{fig:dsl}, a program in this DSL takes as input a question $Q$, keyword(s) $K$, and a webpage $W$, %(represented using the tree representation from Section~\ref{sec:prelim}), 
and it returns a \emph{set} of strings that collectively answer the question.


\begin{figure}[t]
% \vspace{-0.15in}
\footnotesize
\[
\begin{array}{rlll}


{\rm Program} \ \prog ::= & \lambda \question_, \keywordss, \webpage. \{   \guard_1 \rightarrow \lambda x. e_1, \ldots, \guard_n \rightarrow \lambda x.  e_n \} \\ 



% {\rm Guard}  \ \guard ::= & \texttt{ContainsKeyword}(ns, \keywordss, t) \\ 
% | & \texttt{ContainsSection}(ns, \keywordss, t) \\
% | & \texttt{ContainsEntity}(ns, l) \\ 
% | & \texttt{IsSingleton}(ns) \\ 
% | & \neg \guard \\
%\ \ | \ \ \guard \wedge \guard \\ 

{\rm Guard} \ \guard ::= & \texttt{Sat}(\nodeExt, \lambda z. \neural)  \ \ | \ \  \texttt{IsSingleton}(\nodeExt) \\



% {\rm Extractor} \ e ::= &  \texttt{ExtractContent}(x) \\ 
%  | & \texttt{Split}(e, c) \\
%  | & \texttt{Filter}( \lambda z. \phi, e) \\ 
%  | & \texttt{ExtractEntities}(e, l) \\ 
%  | & \texttt{ExtractKeywordMatches}(e, \keywordss) \\ 
%  | & \texttt{ExtractAnswers}(e, \question, k) \\ 


{\rm Extractor} \ \stringExt ::= & \texttt{ExtractContent}(x) \\
| & \texttt{Substring}(\stringExt, \lambda z. \neural, k) \\
| & \texttt{Filter}(\stringExt, \lambda z. \neural)\\
| & \texttt{Split}(\stringExt, c) \\
 
 
% {\rm Predicate} \ \phi :: = & \texttt{HasEntityLabel}(z, l) \\ 
%  | &  \texttt{IsSimilarTo}(z, \keywordss, t) \\ 
%  | & \phi \wedge \phi \ \ | \ \ \phi \vee \phi \ \ | \ \ \neg \phi \\ 
 
% {\rm Node \ Extractor} \ ns ::= & \texttt{GetNodesByKeyword}(\webpage, \keywordss, k, t ) \\ 
%  | & \texttt{GetNodesByQuestion}(\webpage, \question, k) \\ 
%  | & \texttt{GetRoot}(\webpage) \\
%  | & \texttt{GetChildren}(ns) \\ 
%  | & \texttt{GetLeaves}(ns) \\ 
%  | & \texttt{GetStructured}(ns) \\ 


{\rm Section \ locator} \ \nodeExt ::= & \texttt{GetRoot}(\webpage) \\
| & \texttt{GetChildren}(\nodeExt, \lambda n.\nfilter) \\
| & \texttt{GetDescendants}(\nodeExt, \lambda n. \nfilter) \\
 
% {\rm Node \ Predicate} \ \psi ::= &  \texttt{IsList}(x)\\
% | &  \texttt{IsTable}(x) \\ 
% | & \texttt{IsString}(x) \\ 
{\rm Node \  filter} \ \nfilter ::= &  \texttt{isLeaf}(n) \ | \  \texttt{isElem}(n) \\
   | &  \texttt{matchText}(n, \lambda z. \phi, b) \\
| & \top \ \ | \ \ \nfilter \wedge \nfilter \ \ | \ \ \nfilter \vee \nfilter \ \ | \ \ \neg \nfilter \\
{\rm NLP \ predicate} \ \neural ::= &  \texttt{matchKeyword}(z, \keywordss, t) \\
| &  \texttt{hasAnswer}(z, Q) \\
| &  \texttt{hasEntity}(z, l) \\
| & \top \ \ | \ \ \neural \wedge \neural \ \ | \ \ \neural \vee \neural \ \ | \ \ \neg \neural \\



\end{array}
\]
\vspace{-0.2in}
\caption{DSL for \toolname. Here, $c$ denotes a character (e.g., a  delimiter like comma), and $l$ is an entity type (e.g. Person). Also, $k \in \mathbb{Z}$, $b$ is a boolean, $t \in [0, 1]$ is a threshold.}
\label{fig:dsl}
\vspace{-0.2in}
\end{figure}

As shown in Figure~\ref{fig:dsl}, each \dsl program is a sequence of \emph{guarded expressions} of the form $\guard_i \rightarrow \lambda x. \stringExt_i$ where the \emph{guard} $\guard_i$ locates relevant tree nodes and checks whether they satisfy some property, and  the \emph{extractor} takes as input a set of tree nodes (computed by the guard) and returns a set of strings (see Figure~\ref{fig:dsl-types} for their types).
%serves as both locating the relevant node and checking whether the located nodes satisfy a certain predicate, 
% each \dsl program is a sequence of \emph{guarded expressions} of the form $\guard_i \rightarrow \lambda x. \stringExt_i$, where $\guard_i$ is a guard 
%and $\stringExt_i$ is a so-called \emph{extractor} that returns  a set of strings (see Figure~\ref{fig:dsl-types}). 
The program returns the result of  expression $\stringExt_i$ if the corresponding guard $\guard_i$ is true and all previous guards $\guard_1, \ldots, \guard_{i-1}$ evaluate to false.  Intuitively, the guards are used to determine the webpage ``schema''
and locate the relevant tree nodes from which to extract information. Then, the corresponding expression $\stringExt_i$ extracts the relevant text from those nodes. 

In more detail, guards $\guard$ in a \dsl program locate the relevant sections  $N$ of the webpage using so-called \emph{section locators} and check whether nodes $N$ satisfy some predicate. If they do, the located sections $N$ are bound to variable $x$ of the corresponding extractor expression $\stringExt$, and the result of evaluating $\stringExt$ on $N$ is returned. On the other hand, if a guard evaluates to false, then the next guard is evaluated, and this process continues until one of the guards evaluates to true. If all guards evaluate to false, the return value of the program is $\varnothing$. Next, we explain the \dsl constructs in more detail.







\begin{figure}[t]
% \vspace{-0.15in}
\footnotesize
\[
% \begin{array}{cll}
% p & :: \texttt{Question} \times \texttt{Keywords} \times \texttt{Webpage} \rightarrow \texttt{Set<String>} \\ 
% \stringExt & :: \texttt{Set<String>}  \\
% x & :: \texttt{Set<Node>} \\
% z & :: \texttt{String} \\
% n & :: \texttt{Node} \\
% \nodeExt & :: \texttt{Set<Node>} \\ 
% \nfilter, \neural, \guard & :: \texttt{Bool} \\
% \end{array}
\begin{array}{ll}
   \multicolumn{2}{l}{p :: \texttt{Question} \times \texttt{Keywords} \times \texttt{Webpage} \rightarrow \texttt{Set<String>}} \\
    \multicolumn{2}{l}{\guard :: \texttt{Bool} \times \texttt{Set<Node>}} \\
    \stringExt :: \texttt{Set<String>} & z :: \texttt{String} \\
    x :: \texttt{Set<Node>} & n :: \texttt{Node} \\
    \nodeExt :: \texttt{Set<Node>} & \nfilter, \neural :: \texttt{Bool}
\end{array}
\]
\vspace{-0.2in}
\caption{Types of different symbols in the \dsl grammar}
\vspace{-0.2in}
\label{fig:dsl-types}
\end{figure}


\noindent
\paragraph{Pre-trained NLP Models.} Our DSL contains three pre-trained neural models for extracting information from webpages.  These pre-trained models are used inside predicates $\neural$ and include the following primitives:
\begin{itemize}[leftmargin=*]
\item {\bf Keyword match:} Given string $z$, the  $\texttt{\small matchKeyword}(z, K, t)$ predicate evaluates to true if the semantic similarity between  $z$ and  keyword $k$ exceeds  threshold $t \in [0,1]$ for some keyword $k \in K$. 
\item {\bf Question answering:} The   $\texttt{\small hasAnswer}(z, Q)$ predicate returns true if a pre-trained neural network for textual question answering can find the answer to the given question $Q$ in input string $z$. 
\item {\bf Entity matching:} Given string $z$,  $\texttt{\small hasEntity}(z, l)$  returns true if a  neural model for entity matching decides that $z$ contains an entity of type $l$ (e.g., person, location). 
\end{itemize}
These neural primitives draw on standard NLP modeling tools for each of their respective tasks. By using standard tools, we can exploit not only pre-trained vectors \cite{pennington2014glove} and  models such as BERT \cite{bert}, but we can take advantage of training sets created for other tasks like question answering \cite{squad}. This design choice allows us to leverage neural components despite the lack of substantial training data.


%We can therefore use learning-based components despite the few-shot learning scenario we are operating in. 
%Observe that our DSL also allows combining these neural classifiers using the standard boolean connectives, $\land, \lor$, and $\neg$.

% \begin{example}
% \color{red}{Add an example}
% \end{example}

\noindent
\paragraph{Section locators.} Our \dsl DSL includes so-called \emph{section locator} constructs $\nodeExt$ for identifying tree nodes from which to extract information. Section locators allow navigating the tree structure and identifying nodes that satisfy a given predicate. In particular, given a webpage $W$, $\texttt{getRoot}(W)$ returns the root node of the webpage, and the recursive {\tt getChildren} and {\tt getDescendants} constructs return respectively the children and descendant nodes satisfying a certain predicate $\nfilter$. 
Predicates on nodes allow testing whether a given node is a leaf ({\tt isLeaf}), whether it is a list/table element ({\tt isElem}), or whether the text contained in that node matches NLP predicate $\neural$ ({\tt matchText}). Note that the third boolean argument of {\tt matchText} specifies whether to consider only text within that node ($b = \texttt{false}$) or whether to consider the text in the entire subtree ($b = \texttt{true}$).
% \begin{example}
% \color{red}{Add an example}
% \end{example}

\paragraph{Guards.} As mentioned earlier, guards in our DSL are used for locating  relevant sections within a webpage and testing their properties. In particular, a guard $\guard$ uses section locators to identify relevant nodes  $N$ and then checks their properties via the {\tt IsSingleton} and {\tt  Sat} predicates.  As its name indicates, {\tt IsSingleton} tests whether $N$ contains a single node. Intuitively, this predicate is useful because existing textual question answering systems like  {\tt hasAnswer}  are more likely to be effective if the desired information can be found within a single block of text. 
%\xinyu{question answering systems here refer to the ML models? kind of confusing since we are also a QA system?}
%Thus, the  extractor ends up being correlated with whether $N$ is a singleton or not. 
On the other hand, the {\tt Sat} predicate is used to test whether \emph{any} of the nodes $n \in N$ satisfy some neural classifier $\neural$ --- i.e., ${\tt Sat}(N, \lambda z. \neural)$ checks whether  text $z$ of node $n$ satisfies $\neural$ for some $n \in N$. 

% \begin{example}
% \color{red}{Add an example}
% \end{example}



\paragraph{Extractors.} The extractor constructs are used to extract text from relevant sections  $N$ of a webpage. Note that these relevant sections are determined by the corresponding guard and bound to variable $x$ referenced in the extraction construct.  In the simplest case, the {\tt ExtractContent} function returns the string content of each node $n \in N$. The remaining constructs are recursive and allow (a) extracting substrings, (b) filtering elements from a  set, and (c) splitting a string into multiple strings. In particular, ${\tt Substring}(n, \lambda z. \neural, k)$ returns the top-k substrings satisfying neural classifier $\neural$ on $n$'s contents. Similarly, ${\tt Filter}(N, \lambda z. \neural)$ filters those nodes $n$ whose content does not satisfy $\neural$ from set $N$. Finally, ${\tt Split}(n, c)$ generates multiple new substrings by splitting $n$'s content based on the provided delimiter $c$ (e.g., comma). 

% \begin{example}
% \color{red}{Add an example}
% \end{example}

\begin{comment}


\begin{itemize}[leftmargin=*]
    \item {\bf GetNodesByKeyword:} Given webpage $W$ and keywords $K$, this operator locates the top $k$ nodes whose corresponding text is most similar to $K$. This construct computes a similarity score $s \in [0,1]$ using a neural network and returns the top $k$ nodes whose corresponding score is above some threshold $t \in [0,1]$.
 \item {\bf GetNodesByQuestion:} Given a webpage $W$ and question $Q$, this construct returns the top $k$ nodes whose corresponding text best answers the provided question. In more detail, this construct leverages a neural network trained for question answering to produce  a ranked list of answers to the provided question for the entire webpage.  Then, it produces the top $k$ nodes whose corresponding text contains the answer returned by the neural model.
 \item {\bf Tree navigation constructs:} The next three constructs, namely {\tt GetRoot}, {\tt GetChildren}, {\tt GetLeaves}, allow us to navigate the tree structure. In particular, {\tt GetRoot} returns the root node for the webpage; {\tt GetChildren} returns all the children of a given set of nodes, and {\tt GetLeaves} returns all the leaves reachable from the specified nodes. 
 \item {\bf Filtering construct:} The   {\tt GetStructured} construct only retains those nodes that correspond to structured HTML elements (i.e., lists and tables). 
 
\end{itemize}
 Observe that some of these constructs (namely, {\tt GetChildren}, {\tt GetLeaves}, and {\tt GetStructured}) can recursively contain other node extraction operators.



\noindent 
\paragraph{Guards.} As mentioned earlier, guards are used to decide which extractor to use for answering the provided question. Specifically, a guard is a conjunction of literals, where each literal is a predicate  or its negation.   Predicates are applied to the result of a node extractor, and  the DSL provides four types of predicates that we found to be useful:

\begin{itemize}[leftmargin=*]
    \item {\bf ContainsKeyword:} This predicate returns true iff any of its input nodes $ns$ contain text whose similarity score for $K$ is above a certain threshold.  Similar to the node extractor {\tt GetNodesByKeyword}, this predicate is implemented using a neural model for computing semantic text similarity. 
    \item {\bf ContainsSection:} This predicate returns true iff any of its input nodes $ns$ contains a ``section title'' whose similarity score for $K$ exceeds some threshold $t$. In particular, we say that a node $n$ contains a section title $s$ if $s$ is the text associated with an \emph{internal node} reachable from $n$. This construct is also implemented using a neural network.
     \item {\bf ContainsEntity:} This predicate, again implemented by a neural network, returns true iff any of its input nodes given by $ns$ has text containing an entity with label $l$ (e.g., person, date, location).
     \item {\bf IsSingleton:} This predicate returns true iff its input node set $ns$ is a singleton.
\end{itemize}

Intuitively, the neural predicates are used to decide whether the extracted nodes correspond to the relevant sections of this specific webpage for answering the given question. On the other hand, the non-neural \texttt{IsSingleton} construct is useful for determining what type of extractor to use. In particular, since question answering systems are generally better at providing a single answer from a contiguous chunk of text, we found the \texttt{IsSingleton} predicate to be useful for guiding what type of extractor to use. 
%For example, if the task requires merging information from different parts of the webpage, 

\paragraph{String extractors.} The (conditional-free) string extractor constructs in our DSL extract the desired information from a given set of tree nodes (bound to parameter $x$). At a high level, string extractors first obtain all text contained in the input nodes (using the \texttt{ExtractText} construct) and then further refine this text using the other string extraction constructs. In particular, \texttt{Split} splits its input text into a set of strings based on the provided delimiter $c$, and \texttt{Filter} removes some of the elements in the set regarding whether or not its predicate evaluates to true.  The remaining three constructs are all neural and use the same  models described earlier for finding entities, determining keyword similarity, and answering questions. Note that the predicates used inside the \texttt{Filter} construct are also neural and check whether a string contains a certain type of entity or is similar to a given keyword.



\begin{example}

\end{example}


\end{comment}

\begin{comment}

A program $p$ takes as input a question $\question$, and a webpage $\webpage$, and it returns a list of strings where each string corresponds a potential answer to question $\question$. $g$ is a guard and $e$ is an expression that extracts an answer. 

Both $g$ and $e$ use a node localization program $ns$. Let us first explain what $ns$ is. 
$ns$ returns a list of DOM nodes. 
It could be a list of headers in $\webpage$. In this case, the list of headers is obtained by invoking \texttt{GetHeaders} on $\webpage$ which finds the top-$k$ nodes whose content matches keywords in $\keywordss$ with a similarity score greater than $t$. 
We also have a function \texttt{GetNodes} that finds the top-$k$ nodes that correspond to answers to question $\question$. 
\texttt{GetChildren} function returns children of those nodes returned by another node localization program $ns$. Similarly, \texttt{GetLeaves} gives leaves of $ns$. Note that $ns$ combines neural reasoning and symbolic reasoning, where it uses a QA system and keyword matching to locate an initial set of relevant nodes and further leverages the DOM structure to improve the coverage (in case QA is not complete). 

Given a set of relevant nodes, $e$ extracts candidate answers from these nodes. 
In the simplest case, \texttt{ExtractContent} extracts content from a list $ns$ of DOM nodes. 
This content can be further processed using other operators to produce more refined answers. 
For instance, \texttt{Filter} operator keeps only strings in $e$ that satisfy a predicate $\phi$. 
\texttt{ExtractEntities} extracts entities in those strings in $e$ that are labeled with $l$. 
\texttt{ExtractKeywordMatches} extracts any span from strings in $e$ as long as the span matches a keyword in $\keywordss$. 
\texttt{ExtractAnswers} invokes the QA system on each string in $e$ for question $\question$ and keeps the top-$k$ answers for each string. 
\texttt{SplitByComma} splits each string in $e$ by comma. 

On the other hand, the guard $g$ also uses a set of nodes to evaluate whether we localize to the right area. For instance, \texttt{HasEntity} return true if $ns$ contains an entity. \texttt{HasKeywords} return true if $ns$ contains at least one keyword match. \xinyu{Should $g$ use the same $ns$ as $e$? If not, it does not seem to make much sense...} 



\xinyu{We need: 1. an interface for the web QA system 2. a definition of the DOM}

\end{comment}


==> WebExtract arxiv/eval.tex <==
\section{Evaluation}~\label{sec:eval}
In this section, we describe a series of experiments that are designed to answer the following research questions:

\begin{itemize}[leftmargin=*]
    \item {\bf RQ1.} How does \toolname's performance compare against  other question answering and information extraction tools?
    % \todo{Should we modify the research question?}
    \item {\bf RQ2.} How important are the synthesis techniques proposed in Section~\ref{sec:synthesis}?
\item {\bf RQ3.} Is the  program selection technique based on transductive learning (Section~\ref{sec:self-supervision}) useful in practice?
\end{itemize}

\paragraph{Benchmarks} To answer these questions, we evaluate \toolname on 25 different tasks across four different domains, namely   faculty profiles, computer science conferences,  university courses, and clinic websites. For each domain, we collect approximately 40 webpages and evaluate the performance of each tool in terms of $F_1$ score, precision, and recall. For each task, out of around 40 webpages, around 5 of them are used for training (i.e. synthesis) and the remaining is the test set. Table~\ref{tab:task} describes the 25 tasks used in our evaluation.


\paragraph{Experimental Setup} All of our experiments are conducted
on a machine with Intel Xeon(R) W-3275 2.50 GHz CPU
and 16GB of physical memory, running the Ubuntu 18.04
operating system with a NVIDIA Quadro RTX8000 GPU. 

\begin{table}[]
    \centering
    \scriptsize
    \caption{Description of the tasks used in evaluation.}
    \begin{tabular}{|c|l|}
    \hline
    Domain & Description  \\
    \hline
    \multirow{8}{*}{Faculty} & Extract  current PhD students \\
     & Extract  conference publications at PLDI  \\
     & Extract  courses they have taught   \\
     & Extract those papers that received a Best Paper Award \\
     & Extract  program committees they have served on \\
     & Extract  conference papers  they published in 2012 \\
     & Extract  co-authors among all papers published at PLDI \\
     & Extract  formerly advised students \\
     \hline
     \multirow{6}{*}{Conference} & Extract  program committee members \\
     & Extract  program chairs \\
     & Extract the topics of interest  \\
     & Extract the paper submission deadlines \\
     & Extract whether the conference is single-blind or double-blind \\
     & Extract  institutions PC members are from \\
     \hline
     \multirow{6}{*}{Class} & Extract the name of instructors \\
     & Extract the time of the lectures \\
     & Extract the name of teaching assistants \\
     & Extract the date of the exams \\
     & Extract  information about  textbooks \\
     & Extract information on how   grades are assigned \\
     \hline
     \multirow{5}{*}{Clinic} & Extract the doctors or providers \\
     & Extract the provided services \\
     & Extract the types of treatments they specialize in\\
     & Extract the accepted insurances \\
     & Extract the locations \\
     \hline
    \end{tabular}
    \vspace{-10pt}
    \label{tab:task}
\end{table}


\subsection{Comparison with Other Tools}

To answer our first research question, we compare \toolname\ against the following baselines:
\begin{itemize}[leftmargin=*]
\item {\sc BERTQA}~\cite{bert}: This is a state-of-the-art textual question answering system that takes as input an entire webpage and a question and outputs the answer.~\footnote{We also tried fine-tuning this model using the labels in our training examples; however, we do not report results for the fine-tuned model since 
its result is
%the $F_1$ score is 
actually worse compared to ~\cite{bert}.}. 
%This baseline utilizes the same model described in Section~\ref{sec:impl}. \jc{I think we should fine tune the model on our examples a bit just to make this baseline looks a bit more convincing.}
\item {\sc HYB}~\cite{raza2020web}: This is a programming-by-example system that takes a set of webpages as input and synthesizes XPath programs for data extraction. 
%web data extraction programs in a DOM query language (such as XPath). This system is based on a semi-supervised enumeration-based synthesis technique and requires a few example from the user. 
\item {\sc EntExtract}~\cite{liang2014}: This is a zero-shot entity extraction tool for webpages using a natural language query as input. 
\end{itemize}

Note that these baselines do not address \emph{exactly} the same problem addressed by \toolname in that they take fewer inputs. Thus, while our comparison is not completely apples-to-apples, these systems are the closest ones to \toolname for performing a comparison.
 
\begin{figure}
    \centering
    % \input{baselinecomp1}
    \input{baselinecomp2}
    \caption{Comparison between \toolname and other tools }
    \vspace{-10pt}
    \label{fig:baselines}
\end{figure}

\begin{table*}[]
\small
    \centering
    \caption{Evaluation results for each baseline per domain. P stands for Precision and R means Recall.}
    \begin{tabular}{|c|ccc|ccc|ccc|ccc|}
    \hline
    \multirow{2}{*}{Domain} & \multicolumn{3}{c|}{\toolname} & \multicolumn{3}{c|}{{\sc BERTQA}} & \multicolumn{3}{c|}{{\sc HYB}} & \multicolumn{3}{c|}{{\sc EntExtract}} \\
    & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ \\
    \hline
    Faculty & 0.72 & 0.80 & 0.75 & 0.44 & 0.08 & 0.18 & 0.48 & 0.02 & 0.04 & 0.02 & 0.14 & 0.04 \\
    Conference & 0.71 & 0.69 & 0.70 & 0.58 & 0.31 & 0.32 & 0.26 & 0.02 & 0.03 & 0.07 & 0.20 & 0.09 \\
    Class & 0.63 & 0.77 & 0.68 & 0.55 & 0.26 & 0.31 & 0.18 & 0.04 & 0.04 & 0.04 & 0.09 & 0.05 \\
    Clinic & 0.71 & 0.62 & 0.66 & 0.31 & 0.02 & 0.04 & 0.42 & 0.06 & 0.09 & 0.14 & 0.20 & 0.16 \\
    \hline
    \end{tabular}
    \label{tab:domain-results}
\end{table*}

Our main results are summarized in \figref{fig:baselines}, and Table~\ref{tab:domain-results} shows a more detailed breakdown of results across our four domains. As we can see from \figref{fig:baselines}, \toolname outperforms all three baselines in terms of average $F_1$ score, precision, and recall, and, accoring to Table~\ref{tab:domain-results}, these results hold across all four domains.  Among the three other tools, {\sc BertQA} has the best performance; however, it has significantly worse recall and $F_1$ score compared to \toolname. 

\paragraph{Failure analysis for the baselines.} We briefly explain why the baseline systems perform poorly in our evaluation.  As mentioned earlier, a textual QA system like  {\sc BERTQA} fails to take advantage of the inherent structure in webpages and performs particularly poorly on tasks that require extracting multiple different spans from the input webpage. On the other hand, {\sc EntExtract} does leverage the tree structure of the webpage but we found that it often returns irrelevant answers (e.g., publications instead of students). We believe this is because {\sc EntExtract} generates extraction predicates based on XPath queries, but most of our tasks are difficult to solve using simple XPath programs.  Finally, {\sc HYB} tries to synthesize programs that exactly match the provided labels (i.e., perfect $F_1$ score); however, since such programs do not exist for many tasks, synthesis fails in several cases. 

% \red{We find the root cause that these three baselines do not work well in our tasks is that these tools are not designed for this purpose. The point of this evaluation is no means a criticism about these prior techniques but to show that \toolname is able to solve information extraction tasks that are out of scope for prior techniques. }

%However, a couple of our tasks require extracting multiple spans of answers in the webpages. While {\sc EntExtract} baseline is capable of extracting multiple spans of answers from webpages, we found that most of the time it fails to extract the information that is relevant to the natural language. For example, it returns very similar answers for the task ``Extract current PhD students'' and ``Extract conference publications at PLDI''. The {\sc HYB} baseline can only synthesize program when the labels in the training examples provided are the content of a DOM node but not its substrings. This leads to it not being able to synthesize any  program in some of our tasks. In the cases where it can synthesize a program, it only works on those test data where the websites look very similar to the training data since the synthesized program is based on XPath query. 

\paragraph{Failure analysis for \toolname} There are two tasks on which \toolname does not significantly outperform the {\sc BERTQA} baseline. One of these tasks is extracting conference submission deadlines, and the other one is determining whether a conference is double-blind or not. For these two tasks, the program synthesized by \toolname essentially returns the output of the QA model; hence, it does not outperform {\sc BERTQA}.  

%We investigate the cases where \toolname\ does not significant outperforms baselines such as {\sc BERTQA}. The two tasks that fit into this category are the tasks that extract all submission deadlines of a conference and whether the conference is double-blind or single-blind. Note that, since in these two tasks the answers are typically short, a QA system can do well in this scenario. It turns out that the synthesized programs of these two tasks utilize the QA system to extract the answers and that is the reason that they achieve similar performance as the {\sc BERTQA} baseline. The synthesized program for the ``extracting submission deadline"" task also includes another branch that find the submission deadlines using section  header matching. However, since there are many similar keywords such as "abstract submission deadline", "camera ready submission deadline", while this section locator helps increases the recall but also reduces the precision at the same time. 


%The x-axis shows the $F_1$ cutoff values from 0 to 0.9, and the y-axis represents the number of tasks each tool achieves an $F_1$ score greater than that value. \toolname outperforms all the other tools: it is able to achieves an $F_1$ score greater than $0.5$ for all the $20$ tasks proposed, while {\sc BERTQA} has such a performance in only $3$ tasks and the other two baselines achieve such $F_1$ score in none of the tasks. 

\subsection{Evaluation of the Synthesis Engine}
In this section, we describe an ablation study that quantifies the impact of the proposed synthesis techniques from Section~\ref{sec:synthesis}. In particular, recall that our synthesis algorithm incorporates two key ideas--decomposition and pruning based on $F_1$ score. To evaluate the relative importance of these ideas, we consider the following two ablations of \toolname:
\begin{itemize}[leftmargin=*]
    \item \toolnameD: This is a variant of \toolname that synthesizes guards and extractors jointly. In other words, it does not decompose the synthesis problem into two separate guard synthesis and extractor synthesis sub-tasks. %  More specifically, we modify \figref{alg:branch} so that it directly enumerate all possible branch program in the DSL. Note that in this case we are still capable of doing some pruning when if \jc{the synthesizer is expanding guards???}. 
    \item \toolnameP: This variant does not compute an upper bound on the $F_1$ score of partial programs. Thus, it is unable to prune partial programs from the search space. 
    %perform leverages on decomposition but not on pruning out sub-optimal programs using $F_1$ score.
\end{itemize}

The results of this ablation study are presented in \figref{tab:pruning}. Here, the first column shows average synthesis time (in seconds) for all three variants, and the second column shows the average speedup of \toolname over its two ablations. As we can see, both decomposition and $F_1$-based pruning play a significant role in improving synthesis time.  In particular, pruning improves synthesis time by a factor of $3.6$ and decomposition improves it by a factor of $2.4$.  Note that we do not report $F_1$ scores in Table~\ref{tab:pruning} since all variants synthesize the same programs but  differ in how long they take to do so. 

%time it takes for each tool to synthesize the optimal programs on the training set. The second column shows the speedup that \toolname achieves with respect to its variants and the third column shows the variance of the speedup across $20$ tasks. As you can see from the figure, both the techniques contributes to more efficient synthesis. Specifically, \toolname shows on average around $3\times$ speedup compared to \toolnameP and a $2\times$ speedup compared to \toolnameD.

\begin{table}[]
    \small
    \centering
    \caption{Results of the ablation  study. This table shows the average training time and the average speedup that \toolname achieves compared to the other two techniques. }
    \begin{tabular}{|c|c|c|}
    \hline
    Technique & Avg time (s) & Avg Speedup \\ %& Var Speedup \\
    \hline
     \toolname & 419 & -  \\
    {\small \toolnameP} & 1351 & 3.6 \\ %& 1.2 \\
   {\small   \toolnameD} & 931 & 2.4 \\ %& 0.5 \\
    \hline
    \end{tabular}
    \label{tab:pruning}
    \vspace{-0.2in}
\end{table}



\subsection{Effectiveness of the Transductive Learning}
In this section, we investigate the usefulness of the transductive learning technique from Section~\ref{sec:self-supervision} by comparing against two simpler baselines:

\begin{itemize}[leftmargin=*]
    \item {\sc Random}: This baseline chooses uniformly at random one of the optimal programs for the training examples. 
    %with  optimal $F_1$ score on the training examples.
    \item {\sc Shortest}: This baseline   chooses uniformly at random one of the \emph{smallest} programs  (in terms of AST size) that  optimize $F_1$ score on the training examples. 
    
   % implements a simple Occam's razor heuristic commonly used in program synthesis systems. In particular, it  chooses a smallest program in terms of AST size.
    
   % the shortest program with smallest total number of nodes. We break ties by randomly choosing one of the programs. The reason we pick this approach because this is a commonly applied heuristic to select programs.   
\end{itemize}


Recall that the transductive learning technique from Section~\ref{sec:self-supervision} is both intended to reduce variance and produce better-quality results on the test set. Thus, we compared \toolname against two baselines in terms of the following two metrics\footnote{In the experiment, these two metrics are computed based on 20 runs.}.

\begin{itemize}[leftmargin=*]
    \item {Mean:} We report percentage improvement of the transductive learning technique in terms of average $F_1$ score over the two baselines.
   % Note that we perform normalization since the $F_1$ scores range 
    \item {Variance:} We also report  the average reduction in variance.

   % Note that the goal here is to show how each model performs with respect to the best and worst sampled program, and since in each task, the $F_1$ scores of the worst and best program vary a lot, we normalize the $F1$ score w.r.t to its max and min. 
\end{itemize}

As we can see from Table~\ref{fig:self-supervised}, the transductive learning technique dramatically reduces variance and modestly improves average $F_1$ score. Thus, by using our proposed transductive learning technique, \toolname achieves much more stable performance (in terms of the quality of the synthesized programs) compared to these other approaches. 

\begin{table}[]
    \small
    \centering
    \caption{Evaluation of  transductive learning. This table shows the \% of improvement in $F_1$ and the reduction in variance of \toolname  compared to the other two techniques. }
    \label{fig:self-supervised}
    \begin{tabular}{|c|c|c|}
    \hline
      Technique   &  \% Improvement in $F_1$ & Reduction in Variance  \\
      %& Avg Var & Max Var\\
    \hline
    %& 1.4E-07\ & 0.0385\\
    {\sc Random} & 6.0\% & 1550$\times$ \\
    %& 5.7E-05 & 0.0931\\
    {\sc Shortest} & 6.3\% & 1570$\times$ \\
    %&5.5E-05 & 0.0461\\
    \hline
    \end{tabular}
\end{table}

\begin{comment}
We use the following three approaches to select the program from the synthesized programs that is used to extract data on the test set and returned to the user:
\begin{itemize}
    \item {\sc SelfSupervised}: Use the technique proposed in Section~\ref{sec:self-supervision} to select the program.
    \item {\sc Random}: Choose one program randomly.
    \item {\sc Shortest}: Pick the shortest program with smallest total number of nodes. We break ties by randomly choosing one of the programs. The reason we pick this approach because this is a commonly applied heuristic to select programs.   
\end{itemize}
For each task, given the set of programs that achieves the optimal $F_1$ score on the training set, we run each setting $20$ times and obtain the $F_1$ scores of the program that is returned to the user on the test set (noted as $F_{1_{setting}}$, where $setting \in$ \{{\sc SelfSupervised}, {\sc Random}, {\sc Shortest}\}). We then compute the relative improvement in each setting using the formula 
\[
improv(F_{1_{setting}}) = \frac{F_{1_{setting}}
- min(F_{1_{setting}})}{max(F_{1_{setting}})-min(F_{1_{setting}})}
\].

Intuitively, this metric reflects the improvement on $F_1$ score each setting made with respect to the min and max of the $F_1$ score it could possibly achieve on the test set.




We present the summary of the results in \figref{fig:self-supervised}. This table shows the average improvement of $F_1$ and average and max variance across $20$ tasks. In particular, {\sc SelfSupervised} achieves an 30\% increase compared to using the {\sc Shortest} heuristic and improved by 15\% compared to randomly picking a program. Furthermore, using {\sc SelfSupervised} significantly reduces the variance of the program selected by two order of magnitudes compared to the other approaches. 

\end{comment}


\noindent 
\paragraph{Remark.} Appendix C presents additional ablation studies evaluating the impact of the different  input modalities as well as the number of training examples. 


==> WebExtract arxiv/impl.tex <==
\section{Implementation}\label{sec:impl}

 In this section, we provide  implementation details about different components of \toolname.

\paragraph{Parsing.} As explained in Section~\ref{sec:prelim}, \toolname represents each webpage as a tree that captures relationships between text elements on the renderd version of the webpage. Thus, \toolname first parses a given HTML document into our internal representation. To do this, we first extract the DOM tree representation using the \emph{BeautifulSoup4} HTML parser and remove unnecessary elements such as images and scripts. Then, when converting to our tree representation, we follow the standard HTML header hierarchy. In particular, the H1 header corresponds to the root node, and $H_{i+1}$ headers are represented as children nodes of the $H_i$ headers. 

%We wish to process the benchmarks webpages into an intermediary format more suitable for evaluating \toolname. This allows us to eliminate reliance on the DOM and clean the content of the webpages. Additionally, we represent the webpage in a logical hierarchical format where the hierarchy represents the content rather than the hierarchy described by the DOM.

%In order to accomplish this, we first download webpages and process the HTML using \textit{BeautifulSoup4} in order to clean unnecessary elements, for example, images and scripts. We then use the library \textit{turndown} in order to convert the HTML into markdown in order to make the parsing simpler compared to traversing the HTML.

%Afterwards, we parse the markdown to construct the final intermediate format. We respect the structure described by the markdown except when parsing headers, we consider each header to be the parent of the following nodes until another header is found which is above the current header. This final format is represented in a JSON document which describes \textit{webpage tree} for the respective document.

\paragraph{Interactive labeling.} Rather than asking users to directly provide labeled webpages, \toolname
 actually interacts with users and  suggests webpages to label. The goal here is to minimize the number of user annotations while ensuring that the labels achieve good coverage of different schemas in the test set. To do so, \toolname clusters webpages based on various features, including which section locator constructs in our DSL yield non-empty answers, the type of entities contained in the extracted sections, the layout of extracted sections etc. We then identify webpages that are similar to and different from the webpages labeled so far and ask the user to label these additional webpages. In practice, we restrict the number of user queries to at most five. 


\paragraph{Neural modules in the DSL} Our tool leverages several existing natural language processing frameworks and models to implement the neural modules. For QA-related constructs, we use the BERT QA system  \cite{bert} as the underlying model. Specifically, we use the version that has been fine-tuned on the SQUAD dataset\footnote{The link to the model: https://huggingface.co/bert-large-uncased-whole-word-masking-finetuned-squad. }\cite{squad}. We use Sentence-BERT~\cite{sbert} to generate sentence embeddings for keyword similarity,  and we employ  Spacy\footnote{https://spacy.io/. Specifically, we use the ``en\_core\_web\_md'' model.}\cite{spacy2} for named entity extraction and sentence segmentation. Since the keyword matching module requires a real-valued threshold $t \in [0,1]$, our synthesis algorithm discretizes  it  using a step size of $0.05$.

\paragraph{Transductive learning loss. } {Recall that our program selection technique proposed in Section~\ref{sec:self-supervision} is parametrized over a loss function $L(\pi; \mathcal{I}, \mathcal{O})$. In our implementation, we take our loss function to be the Hamming distance between the sets of words extracted by each program. In particular, we use loss function: $L(\pi; \mathcal{I}, \mathcal{O}) = {\tt Hamming}(\pi(\mathcal{I}), \mathcal{O}).$}




% \paragraph{Self-supervision loss. } \jc{Recall that our self-supervised program selection technique from Section~\ref{sec:self-supervision} is parametrized over a loss function $L(\pi; \mathcal{I}, \mathcal{O})$. In our implementation, we take our loss function to be the Hamming distance between the sets of words extracted by each program. In particular, let $f$ be the function that queries the probability of a word $w$ according to the distribution $p(\outputexamples\mid\inputexamples,\examples)$. Let the program $\pi$ yields output $o_\pi$, then, our loss function is:}

% \small
% \[
% L(\pi; \mathcal{I}, \mathcal{O}) = -\sum_{w \in \mathcal{O}} \mathbbm{1}(w \in o_\pi)f(w) + \mathbbm{1}(w \notin
%  o_\pi)(1 - f(w))
% \]
% \normalsize


% \paragraph{Self-supervision loss. } Recall that our self-supervised program selection technique from Section~\ref{sec:self-supervision} is parametrized over a loss function $L(\pi; \mathcal{I}, \mathcal{O})$. In our implementation, we take our loss function to be the Hamming distance between the sets of words extracted by each program. In particular, let $f$ be a function that maps a word $w$ to a real value score $v$ according to the distribution $p(\outputexamples\mid\inputexamples,\examples)$ that we constructed in Section~\ref{sec:self-supervision}  and whether $w$ shows up in the outputs of program $\pi$. If program $\pi_1$ yields output $o_1$ and another program $\pi_2$ yields output $o_2$, then the difference between two programs can be calculated as:
% \small
% \[
% L(\pi_1, \pi_2) = \sum_{w \in o_1 \cup o_2} |f(w, \pi_1) - f(w, \pi_2)|
% \]
% \normalsize


\paragraph{Hyperparameters.} The {\toolname} system has certain hyper-parameters that control the maximum depth of synthesized programs. By default, the hyper-parameter for guard depth is set to $7$ and the one for extractor depth is set to be $5$.  There is also another hyper-parameter (with a default value of $1000$) that controls the number of programs used to construct an ensemble during transductive learning.



==> WebExtract arxiv/intro.tex <==

\section{Introduction}\label{sec:intro}

As the amount of information available on the web proliferates, there is a growing need for tools that can extract relevant information from  websites. Due to the importance of this problem, there has been a flurry of research activity on \emph{information extraction}~\cite{liang2014, lockard20zeroshotceres} and \emph{wrapper induction}~\cite{muslea1999hierarchical, hsu1998generating, chang2001iepad, crescenzi2001roadrunner, anton2005xpath, raza2020web, flashextract, gulhane2011web}. In particular, most recent research from the natural language processing (NLP) community  focuses on unstructured text documents and employs powerful neural models to automate information extraction and question answering (QA) tasks. On the other hand, most  wrapper induction work 
%from the databases community 
focuses on semi-structured documents and aims to synthesize programs (e.g., XPath queries) to extract relevant nodes from the DOM tree. While such wrapper induction techniques work well when the target webpages have a shared global schema (e.g., Yelp pages or LinkedIn profiles), they are not as effective on structurally heterogeneous websites such as faculty webpages. On the other hand, ML-based techniques from the NLP community are, in principal, applicable to  heterogeneous websites; however, by treating the entire webpage as unstructured text, they fail to take advantage of the inherent tree structure of HTML documents. 

In this paper, we propose a new information extraction approach ---based on \emph{neurosymbolic program synthesis} --- that combines the relative strengths of wrapper induction techniques for webpages with the flexibility of neural models for unstructured documents. Our approach targets structurally heterogeneous websites with no shared global schema and can be used to automate many different types of information extraction tasks. Similar to prior program synthesis approaches\cite{fidex, flashextract}, our approach can learn useful extractors from a \emph{small} number of labeled webpages.
% Our approach is based on few-shot learning \cite{fewshot}, so it can learn useful extractors from a \emph{small} number of labeled webpages. 

\begin{figure}
    \includegraphics[scale=0.24, trim=237 500 500 270, clip ]{figure/WebQA-new5.pdf}
    % \vspace{-0.2in}
    \caption{Schematic overview of our approach}
    \label{fig:workflow}
\end{figure}

As illustrated in Figure~\ref{fig:workflow}, our approach takes three inputs, including (1) a natural language query, (2) a small number of labeled webpages, and (3) a much bigger set of unlabeled webpages from which to extract information. For instance, if the task is to extract PhD students from faculty webpages, the input might consist of a question such as ``Who are the PhD students?" as well as keywords like "advisees'' and "PhD students''. In addition, the user would also provide a set of target faculty webpages, together with labels (i.e., names of PhD students) for a few of these. Given this input, the goal of our technique is to generate a program that can be used to extract the desired information from all target webpages.

%The workflow of our proposed approach is shown schematically in Figure~\ref{fig:workflow}. Given a set of structurally heterogeneous  webpages (e.g., faculty webpages), our goal is to extract some information (e.g., list of PhD students) from each input document. To automate this task using our approach, the user provides two types of input consisting of natural language and examples. In particular, the natural language component involves  a question describing the task, such as "Who are this person's PhD students?", as well as some  relevant keywords.  On the other hand, examples include a small number of webpages and the corresponding text to be extracted from each webpage. Given these inputs, our goal is to automatically extract the desired answer for \emph{all} target webpages.
%, including for those whose  schema is different from those labeled by the user.

To solve this challenging problem, we employ a multi-pronged solution that incorporates three key ingredients:
\begin{itemize}[leftmargin=*]
    \item {\bf Neurosymbolic DSL: } To combine the relative strengths of wrapper induction techniques with the flexibility of language models, we design a new neurosymbolic domain-specific language targeted for web question answering. Our DSL combines pre-trained neural modules for natural language processing with standard programming language constructs for string processing and tree traversal.
    %such as conditionals and primitives for navigating the tree structure of HTML documents.
    \item {\bf Optimal program synthesis:} To utilize this DSL for automated web information extraction, we describe a new program synthesis technique for finding DSL programs that best fit the labeled webpages. However, since it is often impossible to find programs that \emph{exactly} fit the provided labels, we instead search for programs that optimize $F_1$ score\footnote{{ $F_1$ score is computed as  $2 \cdot \frac{\texttt{precision} \cdot \texttt{recall}}{\texttt{precision} + \texttt{recall}}$. It is a common evaluation metric in information extraction. }}. Our proposed optimal synthesis method is compositional and leverages   a  monotonicity property of the DSL to aggressively prune parts of the search space that are guaranteed \emph{not} to contain an optimal program.  
    \item {\bf Transductive program selection:} During synthesis, there are often \emph{many} (e.g., hundreds of) DSL programs with optimal $F_1$ score on the labeled data. However, not all of these candidate programs perform well on  test data, and standard heuristics (e.g., based on program size) are not effective at distinguishing between these programs. We address this challenge using transductive learning: it generates \emph{soft labels}  for the test data based on all candidate programs and then chooses the ``consensus'' program whose output most closely matches the soft labels.
    %Even worse, these programs that are both optimal with respect to the training data yield very different $F_1$ scores on unseen webpages in the test data. 
  %  Thus, given a set of candidate programs returned by the optimal synthesis engine, we need to predict the ``best'' program for a new webpage. We solve this problem using a self-supervised learning approach. That is, we generate \emph{soft labels}  for the test data based on all candidate programs, and then, for a given webpage, we choose the ``consensus'' program whose output most closely matches the soft label.% This self-supervised approach allows us to generate a useful \emph{ensemble model} of the hundreds of programs that are returned by the optimal synthesis engine.
\end{itemize}

We have implemented our proposed approach in a tool called \toolname{}
%. Given a query and a set of target webpages, \toolname{} interacts with the user and suggests a small subset of the target webpages to label. Then, once it synthesizes  programs that achieve optimal $F_1$ score on these ``training" examples, it uses self-supervision to select  which program to use to label the  target webpages.
and evaluate it across  several different tasks  and many webpages. Our evaluation demonstrates that \toolname{} yields significantly better results compared to existing baselines,  including both question answering models and wrapper induction systems. We also perform ablation studies to evaluate the relative importance of our proposed techniques and show that all of these ideas are important for making this approach practical.

In summary, this paper makes the following  contributions:

\begin{itemize}[leftmargin=*]
    \item We propose a new technique for web question answering that is based on optimal neurosymbolic program synthesis.
    \item We present a DSL for web information extraction that combines pre-trained NLP models with traditional language constructs for string manipulation and tree traversal.
    \item We describe a compositional program synthesis technique for finding all programs that achieve optimal $F_1$ score on the labeled webpages. Our synthesis algorithm prunes the search space by exploiting a monotonicity property of the DSL with respect to recall.
    \item We present a transductive learning technique for choosing a good program for labeling the target webpages.
    \item We implement our approach in a tool called \toolname{} and evaluate it on 25 different tasks spanning four domains and 160 webpages.
\end{itemize}

==> WebExtract arxiv/macros.tex <==
\newcommand{\assign}{\gets}
\newcommand{\res}{R}
\newcommand{\bestf}{\emph{opt}}
\newcommand{\guards}{G}
\newcommand{\extractors}{E}
\newcommand{\dsl}{{\sc WebQA}\xspace}

\newcommand{\question}{Q}
\newcommand{\keywordss}{K}
\newcommand{\webpage}{W}
\newcommand{\guard}{\psi}
\newcommand{\prog}{p}
\newcommand{\stringExt}{e}
\newcommand{\nodeExt}{\nu}
\newcommand{\neural}{\phi}
% \renewcommand{\dots}{\cdots}
\newcommand{\nfilter}{\varphi}
\newcommand{\fonescore}{s}
\newcommand{\semantics}[1]{\llbracket{#1}\rrbracket}                    
\newcommand{\jc}[1]{\textcolor{red}{\textbf{JC:} #1}}
\newcommand{\greg}[1]{\textcolor{red}{\textbf{GD:} #1}}
\newcommand{\xinyu}[1]{\textcolor{red}{\textbf{XW:} #1}}
\newcommand{\osbert}[1]{\textcolor{red}{\textbf{OB:} #1}}
\newcommand{\aaron}[1]{\textcolor{red}{\textbf{AL:} #1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}

\newcommand{\toolname}{{\sc WebQA}\xspace}
\newcommand{\toolnameD}{\toolname-{\sc NoDecomp}\xspace}
\newcommand{\toolnameP}{\toolname-{\sc NoPrune}\xspace}
\newcommand{\tableT}{{\tt Table}\xspace}
\newcommand{\listT}{{\tt List}\xspace}
\newcommand{\stringT}{{\tt String}\xspace}
\newcommand{\setT}{{\tt Set}\xspace}

\newcommand{\figref}[1]{Figure~\ref{#1}}

\algnewcommand\Input{\textbf{input: }}
\algnewcommand\Output{\textbf{output: }}

\newcommand{\partition}{P}
\newcommand{\examples}{\mathcal{E}}
\newcommand{\examplee}{e}
\newcommand{\worklist}{\mathcal{W}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}



\newcommand{\irule}[2]{\mkern-2mu\displaystyle\frac{#1}{\vphantom{,}#2}\mkern-2mu}


\newcommand{\inputexamples}{\mathcal{I}}
\newcommand{\outputexamples}{\mathcal{O}}
\newcommand{\inputexamplee}{i}
\newcommand{\outputexamplee}{o}

==> WebExtract arxiv/motivating.tex <==
\section{Motivating Example}\label{sec:motivating}

In this section, we present a motivating scenario for  \toolname\  and highlight salient features of our approach.

\begin{figure*}[!t]
\hspace{-15pt}
\begin{center}
    \begin{minipage}[t]{0.63\linewidth}
    \includegraphics[width=0.48\linewidth,trim=180 300 200 20, clip]{figure/janedoe.pdf}
    \includegraphics[width=0.5\linewidth,trim=170 290 170 0, clip]{figure/johndoe.pdf}
    \caption{Sample faculty websites with their program committee information. Correct answers are in blue; the output of a QA model is underlined in red.}
    \label{fig:webpages}
    \end{minipage}
    \hspace{20pt}
    \begin{minipage}[t]{0.30\linewidth}
    \includegraphics[width=1.0\linewidth, trim=200 310 200 0, clip]{figure/robertdoe.pdf}
    \caption{The synthesized program also works on this website; highlighted text are the extracted output.}
    \label{fig:webpages2}
    \end{minipage}
\end{center}

\end{figure*}

% \begin{figure}
%     \centering
    
    
    
% \end{figure}

\noindent
\paragraph{Usage scenario.} Suppose that the PC chair for a conference needs to form a program committee, and she has access to the websites of many researchers. To help her form a good committee, she wants to extract program committees that each researcher has served on (which is often available on their websites). Since there are too many websites, extracting this information manually is too laborious. 
%On the other hand, it is feasible for the PC chair to provide the desired information for only a small number of webpages.  
Our proposed system, \toolname, is useful in scenarios like this
that require collecting information from many structurally heterogeneous websites. % and where the user is willing to provide a few training examples.


%and  where the desired information may not correspond to  a single  contiguous block of text. 

%On the other hand, automated tools for information extraction and question answering do not work well for this~task. 
%For example, wrapper induction techniques~\cite{tbd} fail to extract any information due to the lack of a shared schema across different websites, whereas  state-of-the-art QA systems (e.g., based on BERT~\cite{bert}) return \emph{some} answer but it is often either not complete or provides the wrong information (e.g., students instead of program committees).
%\osbert{Is the multitude of schemas a fundamental problem for wrapper induction? I believe techniques like FlashExtract can handle a small number of different schemas (using a similar top-level decision list like the one we have). I thought the main challenge would be the need for things like approximate matching.}
%\osbert{Can we tie these shortcomings back to the concrete examples in Figure 2? I would present the figure before this text.}

%Our proposed system, \toolname, is useful in scenarios like this  that require collecting information from structurally heterogeneous websites and  where the desired information may not correspond to  a single  contiguous block of text.  

To use \toolname, the user starts by providing a question (e.g., ``Which program committees has this researcher served on?'') and a set of keywords (e.g., ``PC'', ``Program Committee'', ``Service''). Then, given a target set of websites, \toolname\ asks the user to provide labels for a small number of webpages. For instance,  Figure~\ref{fig:webpages} presents two (hypothetical) websites that \toolname may show to the user, with the user-provided labels highlighted in blue. Observe that both of these webpages are semi-structured in the sense that they contain clearly-delineated sections (e.g., Students, Service); however, they differ both in terms of their high-level structure and what information they contain. 

%\osbert{Maybe we should say here that the program we synthesize gets perfect (training) accuracy, and we discuss test set generalization below.}\xinyu{Re Osbert: I don't quite get what you mean here: perfect accuracy on train set is a bit confusing to me? does that mean 100\% accuracy or just highest accuracy? also, it seems to early here to discuss that.}

\paragraph{Limitations of existing approaches.} We now use this simple motivating example to illustrate why existing approaches are not effective for this type of tasks. As mentioned in Section~\ref{sec:intro}, there are two classes of techniques, namely \emph{program induction} and \emph{question answering}, that could potentially be useful in this setting. 

Like our approach, program induction techniques aim to extract information from webpages based on a small number of user-provided training examples~\cite{raza2020web,iyer2019synthesis}.  Specifically, given a few  labeled webpages, these techniques learn XPath expressions to locate  relevant nodes in the DOM tree. However, as illustrated in Figure~\ref{fig:webpages}, researcher webpages typically do not have a uniform structure. Furthermore, even for webpages that are structurally somewhat similar, they exhibit minor variations (e.g., different section names, relative ordering of sections etc.) that make it very difficult to learn XPath expressions that   generalize well to unseen websites. In addition, almost all existing techniques in this space focus on extracting relevant nodes in the DOM tree; however, they do not attempt to perform any further text processing within that node. 
As illustrated by both webpages in Figure~\ref{fig:webpages}, extracting the desired information requires further processing at the text level, such as extracting relevant substrings. 


An alternative approach for automating this task is to use a state-of-the-art question answering (QA) system that treats the entire webpage as a raw sequence of words.
%In particular,  
%a QA system treats the entire webpage as a raw sequence of words and returns an answer to the provided question. 
%we could in principle treat the entire webpage as a raw sequence of words and use a QA system to answer the provided question. 
However, in practice, such approaches perform poorly since they are not designed to leverage the tree structure of the document. 
Furthermore, because they treat  text across different DOM nodes as natural language,  they have difficulty dealing with more structured information like long comma-delineated lists or formatting with parentheticals. 
%Even pre-trained transformer models have not seen this kind of sophisticated formatting frequently and do not treat its structure appropriately.
For instance, for the two webpages from Figure~\ref{fig:webpages} and the question ``Which program committees has this researcher served on?'', a BERT-based QA system~\cite{bert} yields the suboptimal answers underlined in red in Figure~\ref{fig:webpages}. In particular, it either outputs incorrect spans or includes  text that should not be part of the answer (e.g. ``POPL'20 (SRC)'' in the second webpage). 


%(i) In principle, we could remove the structure and feed the raw sequence of words in the webpage to an machine-learning based technique such as a question-answering (QA) system. However, these techniques perform poorly since they cannot leverage the tree structure of the document. Alternatively, we cannot train a model from scratch on our data since we only have a small number (5-10) labeled examples, which is too few to learn from.

%(ii) In addition, our tasks often require string processing to extract the desired information. For instance, the two webpages from Figure~\ref{fig:webpages} indicate the nature of the activity (e.g., PC, ERC) in parentheses, and different activities are comma separated in the first webpage. This poses several challenges to state-of-the-art QA systems. First, they are based pretrained language models and cannot understand novel words such as ``PLDI'' and ``PC'' that occur very rarely (or not at all) in the training data. Second, most existing QA systems extract a contiguous span of the original text, and would be unable to filter out specific substrings.

% - Technique that requires training to work on the new domain: lack of training data in our setting
% - QA System that doesn't require new training data: 
%  - has difficulty dealing with large documents 
%  - existing qa system can only extract a contiguous chunks of text
%  - 


\begin{comment}

%Such  structural heterogeneity  across different websites  makes it difficult to extract the desired information based purely on the tree structure of the webpage.
%\osbert{Figure 2 is very hard to read, and it's not at all clear that we're looking at webpages. Can we give some more context (e.g., more of the webpage)? Also, why isn't OOPSLA'19 highlighted in the top webpage?}
Observe the following salient features of this example:
\begin{itemize}[leftmargin=*]
\item Both of these webpages are semi-structured in the sense that they contain clearly-delineated sections (e.g., Students, Service); however, they differ both in terms of their high-level structure and what information they contain. Such  structural heterogeneity  across different websites  makes it difficult to extract the desired information based purely on the tree structure of the webpage.

%two websites have globally different schemas and differ significantly in terms of the information they contain. The first webpage lists all the information using header and lists, while the second webpage presents the information using a table. Also, the section "Recent Publications" and "Students" is presented before "Professional Services" while the second webpage does not contain the first two sections. Furthermore, even if we focus on the relevant portions of these webpages, they still present the relevant information in different ways. The first webpage divides profession services into current service and service done in the past; while the second webpage put all the committee information as one long chunks of text.  Thus, the structurally heterogeneous  nature of these websites makes it difficult to extract the desired information based purely on the tree structure of the webpage. \osbert{Have we defined ``schemas''? We are using this word a lot, and it's not clear exactly what it means. Also, more concrete examples would be better.}
\item The desired information does not appear as one contiguous block of text in the first webpage. Part of the PC information is shown under the "Current" and the other parts are presented under "Past". Since most existing QA systems can   extract a contiguous span of the original text, they often have low recall on the types of information extraction tasks that we consider in this paper.
%\osbert{This sounds like a limitation of current implementations, not a fundamental limitation. We could in principle design BERT systems that output more structured responses; we just haven't because focusing on spans is easier.}
\item Some amount of string processing is  needed to to extract the desired information from these webpages. For instance, the two webpages from Figure~\ref{fig:webpages} indicate the nature of the activity (e.g., PC, ERC) in parantheses, and different activities are comma separated in the first webpage. 
\end{itemize}
%\osbert{In general, I think we have neither justified why pure ML fails nor have we justified why pure PL approaches fail. For pure PL, we should really just point out that there are minor differences in section headers, etc. that are hard to deal with using a purely logical approach. For pure ML, we can say that ML has difficulty dealing with large documents, since it cannot exploit the high-level structure (Greg: Do you think this is fair?). Thus, it makes a lot of mistakes.}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \begin{align*}
        & {\tt GetLeaves}({\tt GetSection}(\webpage, \lambda z. {\tt matchKeyword}(z, \keywordss, 0.9)))
        % & {\tt GetChildren}({\tt GetDescendents}({\tt GetRoot}(\webpage), \lambda n. {\tt matchText}(\\
        % & \ \ \ \ \ \ n, \lambda z. {\tt matchKeyword}(z, \keywordss, 0.9), \bot)), \lambda n. {\tt isLeaf}
        % (n))
        \end{align*}
         \caption{Section Locator. $\webpage$ is the input webpage, $\keywordss$ represents the list of keywords}
        \label{fig:sampleprog_locator}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \begin{align*}
         &\lambda x. 
         {\tt Filter}({\tt Split}({\tt ExtractContent}(x),  `,'), \\
         &\lambda z. {\tt matchKeyword}(z, K, 1.0))
    \end{align*}
    \caption{String extractor. We substitute the variable $x$ with  the output of the section locator.}
    \label{fig:sampleprog_extractor}
    \end{subfigure}
    
    \caption{A sample program that works for webpages in \figref{fig:webpages}}
    \label{fig:dsl-program}
\end{figure}

\end{comment}

\paragraph{Key idea \#1: Neurosymbolic DSL} Our approach combines the relative strengths of machine learning and program induction techniques by synthesizing programs in a neurosymbolic DSL for web information extraction.  In particular, our proposed DSL incorporates both pre-trained neural models for question answering, keyword matching, and entity extraction with standard programming language constructs for string processing and tree navigation.  The tree navigation constructs allow taking advantage of webpage structure, while making it possible to handle minor variations (e.g., exact section names) using pre-trained neural models. Furthermore, the presence of string processing constructs in the DSL allows our method to extract fine-grained information within individual tree nodes. 

In more detail, a program in our DSL is structured to first locate relevant nodes in the tree representation of a webpage (see Figure~\ref{fig:webtree}) and then perform additional information extraction from each tree node.  For example, the following  code snippet in our DSL can be used to locate the relevant parts of the webpages from Figure~\ref{fig:webpages}:
{
\small
\begin{align*}
         & {\tt \small GetLeaves}({\tt \small GetDescendents}(r, \lambda z. {\tt \small matchKeyword}(z, \keywordss)))
        \numberthis \label{eq:locator1}
     %   & {\tt GetDescendents}({\tt GetDescendents}(r, \lambda n. {\tt matchText}(\\
        % & \ \ \ \ \ \ n, \lambda z. {\tt matchKeyword}(z, \keywordss), \bot)), \lambda n. {\tt isLeaf}
        % (n))
\end{align*}}
\normalsize
\begin{figure}[t]
    \centering
    \includegraphics[width=0.43\textwidth, trim=400 200 200 50, clip]{figure/webtree.pdf}
    % \vspace{-0.3in}
    \caption{Tree representation of top webpage from Figure~\ref{fig:webpages}. Each node contains the node id, type and its content.}
    \label{fig:webtree}
\end{figure}

Here, $r$ is the root node of the input webpage, and the construct {\tt GetDescendants}($r, \phi$)  returns all tree nodes whose content satisfies predicate $\phi$. In the code snippet above, the predicate $\lambda z. \texttt{matchKeyword}(z, K)$ is implemented by a neural network  that has been pre-trained for keyword matching. Thus, this program first locates all tree nodes whose content matches any of the provided keywords $K$ and returns all of their leaf nodes. For example, given the tree  in Figure~\ref{fig:webtree} representing the top webpage from \figref{fig:webpages}, the {\tt GetDescendants} sub-program will match node $11$, and {\tt GetLeaves}\footnote{Actually, there is no explicit {\tt GetLeaves}(v) construct in our DSL; this is just syntactic sugar for {\tt GetDescendants}(v, $\lambda$ n. {\tt isLeaf}(n)). } will return  nodes $14$ and $15$, which are  leaf nodes of the subtree rooted at node $11$. For the webpages in Figure~\ref{fig:webpages}, this program yields the tree nodes annotated using black boxes. 

Next, given the tree nodes returned by the above code snippet, we can extract the desired information from these nodes using the following code snippet in our DSL: 
\small
\begin{align*}
         &\lambda x. 
         {\tt GetEntity}({\tt Filter}({\tt Split}({\tt ExtractContent}(x),  {\tt COMMA}), \\
         & \qquad \qquad \qquad \qquad \qquad \qquad \lambda z. {\tt matchKeyword}(z, K)), {\tt ORG}) \numberthis \label{eq:extractor1}
\end{align*}
\normalsize
In particular, this code snippet first retrieves the content of tree node $x$ using  {\tt ExtractContent}  and then splits it into a set of (comma-separated) strings using {\tt Split}. Then, it filters those elements that do not match the provided keywords and finally extracts substrings that correspond to an organization entity\footnote{{Note that there is no explicit ${\tt GetEntity}$ on our DSL; this is a syntactic sugar for ${\tt Substring}(e, \lambda z. {\tt hasEntity}(z, {\tt ORG}), 1)$.}}. Thus, assuming sufficiently good neural models for keyword matching and entity recognition, the output of this program would be exactly the highlighted text for the webpages from Figure~\ref{fig:webpages}.
%\xinyu{First of all, I assume this code snippet is run for each of the extracted node (so x is bound to each node of those extracted nodes?) It is slightly strange that we are applying the keyword matching functionality again here, since we applied it once already (this is the same set of keywords, right?) it may also be good to elaborate on why we use organization here (because committees are orgainzations?)}


It is worth noting that the extraction logic described above generalizes fairly well across websites with quite different layouts. In particular, the same DSL program can be used to extract the desired information from Figure~\ref{fig:webpages2} even though this webpage looks quite different from those in Figure~\ref{fig:webpages}. 
% \xinyu{I wonder if it's good to actually show the extraction result for this page (show some boxes). I would be curious to see this when reading here.}


\begin{comment}
combines programmatic tree navigation and string manipulation primitives with pre-trained neural models that are useful for deciding whether some text is relevant for the task at hand. In particular, even though these two webpages are quite different (as explained above), we can still extract the relevant information using a single uniform program in our DSL. In particular, the program  shown in Figure~\ref{fig:dsl-program} can extract the relevant information from both pages in the following way:

\begin{itemize}[leftmargin=*]
\item First, it locates the relevant section (i.e., internal node in the corresponding tree representation) by using a pre-trained neural model (e.g.,  keyword matching). Since both webpages contain a section whose title is a reasonable match with the provided keywords/question, this program is  able to identify the relevant part of the webpage from which to extract information. \osbert{This goes along with what I said above, but we might need to justify why it's fine to use ML for this part but not for the whole task.}
\item Next, the DSL program extracts leaf nodes of this subtree. Since the first webpage contains meta-information (current vs past service) that is not relevant for the target task, retrieving only the leaf nodes discards this irrelevant information for the first webppage while not losing information relevant for the second webpage.
\item Finally, the program from Figure~\ref{fig:dsl-program} refines the extracted text by using a combination of string processing constructs and neural primitives. In particular, it splits the text into a list of (comma-separated) substrings and then filters out those list elements based on similarity with the provided keywords.  
\end{itemize}
\end{comment}

% \begin{figure}
%     \centering
    
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth, trim=130 420 200 0, clip]{figure/janiedoe.pdf}
%     \caption{A sample webpage that \figref{fig:dsl-program} does not work well on.}
%     \label{fig:webpages3}
% \end{figure}

%Beyond extracting the relevant information from the webpages shown in Figure~\ref{fig:webpages}, please observe that this program also generalizes to the websites shown in Figure~\ref{fig:webpages2} even though it looks different from those in Figure~\ref{fig:webpages}.


\paragraph{Key idea \#2: Allowing imperfect solutions.} In our example so far, we were able to find a DSL program that produces exactly the highlighted text from examples in Figure~\ref{fig:webpages}. However, suppose that the pre-trained network for entity extraction is unable to recognize computer science conference names as organizations. In that case, the output of the extraction program from Eq.~\ref{eq:extractor1} would not exactly match the user-provided labels.  In fact, there is \emph{no} program in our DSL that would produce exactly the desired output.  %Nevertheless, despite not being perfect, there are reasonable programs that  provide useful information to the user. For example, consider the following code snippet, which is a sub-program of Eq.~\ref{eq:extractor1}: 
%\xinyu{not sure if i understand completely what this paragraph is saying, but my thought is that the reason we allow imperfect solution should be that the DSL may not contain a program that produce exact match. This message doesn't come across to me from this paragraph (this paragraph is saying, suppose this, then our previous program no long works, but here we have another program that's better but still not perfect, so we should allow imperfect solutions)} 
%xinyu{Further elaboration on my comment: I think we should say something like this: blablab. In that case, the output of theextraction program from Eq. 2 would not exactly match theuser-provided label for the two training examples. In fact, there is no program in our DSL that can perfectly match the user provided examples. However, our DSL still contains some programs that are useful although not perfect. For instance, blabla.}

%\small
%\begin{align*}
 %        &\lambda x. 
 %        {\tt Filter}({\tt Split}({\tt ExtractContent}(x),  {\tt COMMA}), \\
 %        & \qquad \qquad \qquad \qquad \qquad  \lambda z. {\tt matchKeyword}(z, K)) \numberthis \label{eq:extractor2}
%\end{align*}
%\normalsize

%The output of this program \emph{almost} matches the highlighted text except that it will contain an additional ``{\tt (PC)}''. Since such a solution is still useful despite not being an exact match, our method allows such imperfect solutions. 


To deal with this difficulty, our synthesis algorithm aims to  find programs that maximize $F_1$ score  rather than looking for solutions that exactly match the user-provided labels. Thus, we frame our problem as \emph{optimal program synthesis}, where the goal is to find programs that maximize some optimization objective ($F_1$ score in our case). This optimality requirement makes the synthesis problem harder because we need to exhaustively explore the search space. 

\paragraph{Key idea \#3: Transductive learning.} An additional difficulty in our context is that there may be hundreds or even thousands of optimal solutions for a  synthesis task. In particular, given the scarcity of training examples, many different DSL programs  yield the same $F_1$ score on the labeled webpages. For instance, for the two webpages from \figref{fig:webpages}, there are actually $85$  optimal DSL programs that achieve the same $F_1$ score. 
%To gain some intuition about why this is the case, consider the {\tt matchKeyword} construct in our DSL. In reality, this construct takes an additional argument $t \in [0,1]$ that is used as the decision boundary for keyword matching. 
%That is, the implementation of  {\tt matchKeyword}  first generates word embeddings using a neural network and then computes cosine similarity. If the cosine similarity is above the provided threshold, the input text is considered to be a match with the keyword. 
%Since there are many different threshold values that produce the same output on the training examples, the number of solutions to the optimal synthesis problem ends up being quite large. Furthermore, even if we restrict ourselves to a single threshold value for the neural DSL constructs, one can still find a large number of programs that achieve the same optimal $F_1$ score on the few training examples. 
Existing  techniques in the synthesis literature deal with the under-constrained nature of input-output examples by using heuristics to distinguish different candidate solutions. However,  standard heuristics (e.g., based on AST size) do not work well in our setting because there are still \emph{many} programs that are tied with respect to such  heuristics. 

Our approach deals with this challenge using \emph{transductive learning}. In particular, 
given all programs that yield optimal $F_1$ score on the labeled data, it generates \emph{soft labels} for unlabeled webpages by running these programs on the unlabeled webpages and aggregating their outputs. 
%generates \emph{soft labels} for the unlabeled webpages by aggregating over the outputs of all  programs that yield optimal $F_1$ score on the training examples.
Then, among these programs, we choose the one whose outputs most closely match the soft labels for the unlabeled webpages.  In other words,  transductive learning  allows our method to utilize the unlabeled data to choose a most promising program and obviates the need for complex hand-crafted heuristics. 










%To deal with this difficulty, our synthesis algorithm allows imperfect solutions. That is, rather than insisting on an exact match, our method aims to find programs that maximize $F_1$ score, which is a common metric used for evaluating information extraction tasks. Note that this quantitative synthesis problem is a strict generalization of standard program induction (which would require an $F_1$ score of 1 in our setting). Thus, our approach formulates the synthesis task in terms of optimizing an a quantitative objective (i.e., $F_1$ score) rather than requiring an exact match with the user-provided labels. \osbert{Should this come up front, where we describe the PC chair's problem? We can say she doesn't need a perfect solution (and it's impossible to get a perfect solution).}

\begin{comment}

\begin{figure}
    \centering
    \begin{align*}
    & {\tt Locator}_1: {\tt GetRoot}(\webpage)\\
    & {\tt Extractor}_1: \lambda x. {\tt Substring}({\tt ExtractContent}(x), \\ 
    & \qquad \qquad \qquad \lambda z. {\tt hasAnswer}(z, Q), 1)\\
    & {\tt Locator}_2: {\tt GetChildren}({\tt GetDescendents}({\tt GetRoot}(\webpage), \\  
    & \ \ \ \ \ \  \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \lambda n. {\tt matchText}(  n, \lambda z. {\tt hasAnswer}(z, Q), \bot)), \lambda n. \top)\\
    & {\tt Extractor}_2: \lambda x. {\tt ExtractContent}(x)
    \end{align*}
    \caption{Two programs that work on \figref{fig:webpages3}.}
    \label{fig:dsl-program2}
\end{figure}



Of course, the program shown in Figure~\ref{fig:dsl-program} does not generalize to \emph{all} academic webpages. Thus, to get enough coverage, \toolname \ may ask the user to label additional webpages. For example, Figure~\ref{fig:webpages3} shows a webpage for which the program from Figure~\ref{fig:dsl-program} does not return a useful answer. Thus, \toolname  allows combining different types of extraction logic by automatically synthesizing \emph{guards} that determine which extraction logic is most appropriate. For example,
Figure~\ref{fig:dsl-program2} shows two different extraction mechanisms that are suitable for the webpage from  Figure~\ref{fig:webpages3}. In particular, one of them directly invokes the question answering model to get the desired answer, whereas the other one identifies the  relevant tree node using the QA model and then returns all of its children. Finally, to differentiate between the types of webpages shown in Figure~\ref{fig:webpages} and those in  Figure~\ref{fig:webpages3}, \toolname also synthesizes this guard:

\vspace{-5pt}
\begin{align*}
    {\tt AnySat}({\tt L}, \lambda z. {\tt matchKeyword}(z, \keywordss, 0.9))
\end{align*}

where {\tt L} is the section lcoator in \figref{fig:sampleprog_locator}. Thi guard checks whether the leaf nodes in the relevant section contain a match with the keyword. If this guard evaluates to true, then the synthesized program executes the extraction logic from Figure~\ref{fig:dsl-program}; otherwise, it uses one of the extractors from Figure~\ref{fig:dsl-program2}.


While the discussion so far highlights the design choices behind our neurosymbolic DSL, there are two additional considerations that make our synthesis problem uniquely challenging. First, due to the noisy nature of information extraction problems, it may not be possible to find \emph{any} DSL program that \emph{exactly} matches the user-provided labels. Thus, unlike many other programming-by-example and program induction efforts~\cite{crap}, our method must tolerate \emph{imperfect} solutions, as extracting some \emph{useful} information is often preferable over not extracting any information at all. Thus, rather than insisting on an exact match with the user-provided labels, our method aims to find programs that maximize $F_1$ score, which is a common objective function for information extraction tasks. Note that this quantitative synthesis problem is a strict generalization of standard program induction (which would require an $F_1$ score of 1 in our setting). Thus, our approach formulates the synthesis task in terms of optimizing an a quantitative objective (i.e., $F_1$ score) rather than requiring an exact match with the user-provided labels. \osbert{Should this come up front, where we describe the PC chair's problem? We can say she doesn't need a perfect solution (and it's impossible to get a perfect solution).}


An additional synthesis challenge in our setting is that there are \emph{many} programs (often in the order of hundreds) that maximize our optimization objective, but it is hard to choose between them.
\osbert{We should say why: the reason is we have very few labeled examples.}
For example, simple heuristics such as choosing the simplest/shortest program often do not work well in this setting. For instance, consider the two extractors shown in Figure~\ref{fig:dsl-program2}. Here, even though the program that directly invokes the QA model seems much simpler, the alternative program actually generalizes better to other webpages.~\footnote{This is the case because QA models ???} Even worse, since the neural models use a threshold for their classification boundary, many of the synthesized programs may only differ in terms of the constants used. Thus,  it is difficult to manually craft a heuristic for choosing the ``best" program in this context.

Our synthesis technique deals with this challenge by using \emph{self-supervision}.
\osbert{Again, we should tie this back to the example: the PC chair can use this technique because she gathered all the unlabeled examples beforehand. The expensive part is labeling the examples, not gathering them.}
As mentioned in Section~\ref{sec:intro}, we aggregate over the outputs of the synthesized program to generate soft labels for each webpage in the test set and choose the program whose output is the most similar to these soft labels. Thus, such self-supervision  allows our method to utilize the unlabeled data to choose the most promising program and obviates the need for complex hand-crafted heuristics. 
 \end{comment}


\begin{comment}
Our synthesizer takes the 5 labeled examples, along with the question and the keywords, as inputs and returns a set of programs in 8 minutes that achieve the highest $F_1$ score on the training data. One of the sample programs are shown in \figref{fig:synthesized_prog}. At a high level, this program consists of two branches of the form ${\tt Eval}(\guard, \stringExt)$ where the guard $\guard$ first locates the sections that contain the relevant information and checks if these sections satisfy certain predicate, and it categorized the input to the branch that its guard outputs True. The extractor $\stringExt$ extract texts from the contents of nodes located through $\guard$.  One important feature of \toolname\ program is that it contains a combination of neural and symbolic modules where neural modules help find the information from a semantic perspective and symbolic modules help find the information by navigating through the structure of webpages. Neural constructs in this program include word vector similarity ({\tt matchKeyword}), and named entities ({\tt hasEntity}). The reason that we use neural components here is because it better captures the semantic of the information on the web. While "Program committee" seems to be a good keyword and should achieve exact match on a lot of faculties website, it fails on variations of the word that expresses same idea such as "Programme committee", "Committee served as members", "committee members" and etc. Here we briefly explain what this synthesized program is doing: the first branch only looks for the leaves of those sections that contains keywords with similarity threshold more than 0.9, and extract those contents in the located nodes that contains ORG entities. The second branch takes all the leaves of the input document, split all the content by comma if necessary (if the content satisfies a comma-separated-string pattern, no split otherwise) and find out those strings that contains the given keyword.

Unfortunately, this is not the only program that achieves the highest $F_1$ score on the training data. 
%In fact, for the first branch, there are 26 possible guards and 208 possible extractors and in the second branch there are 2 candidate guards and 4 extractors. 
In fact, we end up with a total of 832 candidate programs and it is not entirely clear which one to use. Although these programs work equally well on the training set, their performance varies a lot when applied to new websites --  the best program achieves an $F_1$ score of 0.85 on a held-out test set of pages we annotated, and the worst program achieves an $F_1$ score of 0.62. If we randomly sample a program from it, we will get an average $F_1$ score of 0.75 and if we apply the ``Occam's razor'' principle and picking the shortest program, we will end up with a program of $F_1$ score of 0.78. Although these two approaches return some programs that is better than the worst case scenario, they also brings a lot of variance and therefore greatly affect user experience. 

The key challenge then is that given all these programs that achieve the best $F_1$ score on the training data, we want to select one program to perform extraction on the test data. Our idea here is to pick the program that is closest to the ensemble of the candidate programs. An ensemble is a combination of predication output from different models and in our context, the set of candidate programs voting for the extracted outputs form an ensemble. The intuition here is that these 834 programs will do different things on the test data. However, if we assume that they make independent errors, the ensemble of these  program achieve better performance \red{compared to what???} \cite{?}. To pick the program that is closest to the ensemble, \toolname\ proposes a self-supervision technique that first predict ``soft labels'' for the unlabeled webpages in the held-out test set, and then select the program that performs best according to these soft labels with respect to a given loss function. 

% The intuition here is that these 834 programs will do different things on the new data. However, if we assume that they make \emph{independent} errors, the ensemble of these programs would do well \cite{?}. Since it would be computationally inefficient to run all the programs everytime with new incoming webpages, instead we want to select a single program whose performance is the closest to that of the ensemble. 

Our tool then runs the self-supverised program selection engine, pick the best program and returns the program and the extracted results for all the provided webpages in 20 mins. It returns the program shown in \figref{fig:synthesized_prog} with the $F_1$ score 0.82 on the held-out test set. 

Besides finding out the program committees the faculty has served, \toolname\ can handle a varieties of queries such as "Who are the current PhD students", "Which paper has won the best paper award", and etc. 
\end{comment}

==> WebExtract arxiv/prelim.tex <==
\section{Preliminaries}\label{sec:prelim}

In this section, we discuss how we represent webpages as trees.
%Since our domain specific language for web question answering relies on a specific tree representation,  we introduce our \emph{webpage tree} data structure  and define terminology that we will use in the remainder of the paper. 
Our   representation is different from the standard Document Object Model (DOM) and represents the nesting relationship between {text} elements on the \emph{rendered} webpage to better facilitate web question answering.

\begin{definition}{\bf (Webpage)} A \emph{webpage} is a tree $(N, E, n_0)$ with root node $n_0 \in N$, nodes $N$ and edges $E$. An edge is a pair $(n, n')$ where $n$ is the parent of  $n'$, and each node is  a triple $({\rm id}, {\rm text}, {\rm type})$ where  text is the string content of that node and ${\rm type} \in \{ \emph{list}, \emph{table}, \emph{none} \}$ indicates whether the node corresponds to an HTML list, table, or neither. 
\end{definition}

%Every node $n$ in our tree representation corresponds to an HTML element that contains some text. 
Intuitively, an edge $(n, n')$  indicates that
the text of node $n$ is the header for that of node $n'$ --- i.e., text of $n'$ is nested inside that of $n$ on the rendered version of the webpage. For instance, given an HTML document with title ``Title" and body text ``Text", our representation introduces an edge $(n, n')$ where $n$ has text ``Title'' and $n'$ contains ``Text". 
 
In our  representation, internal nodes can represent structured HTML elements like lists (both ordered and unordered) as well as tables. 
%We refer to such internal nodes as having \emph{structure} and use a predicate \emph{isStructured}($n$) to denote that $n$ represents an HTML list or table.
%\[
%\emph{isStructured}(n) \Leftrightarrow n.{\rm type} \neq \emph{none} 
%\]
For a node $n$ representing an HTML list (resp. table), $n$'s children correspond to elements in the list (resp. rows of the table). 
%Similarly, if a node $n$ represents an HTML table, then $n$'s children denote rows of that table. 
\begin{example}
Our method represents the first webpage in \figref{fig:webpages} as the tree shown in \figref{fig:webtree}. 
%Note that the hierarchy of the tree corresponds to the hierarchy  of the section and the list elements are parsed as nodes of the type list. 



\end{example}

==> WebExtract arxiv/related.tex <==
\section{Related Work}\label{sec:related}

\paragraph{Program synthesis for webpages}

There is  a large body of prior research on learning extraction rules from HTML documents.
In data mining, this problem is known as \emph{wrapper induction}~\cite{kushmerick1997wrapper}, 
%and the goal is to learn extraction rules from HTML pages given a set of manually labeled training examples.
and there is a wide spectrum of proposed solutions~\cite{muslea1999hierarchical, hsu1998generating, chang2001iepad, crescenzi2001roadrunner, anton2005xpath, raza2020web, flashextract, gulhane2011web}.  
For instance, \textsc{Vertex}~\cite{gulhane2011web} uses an \emph{apriori} style algorithm~\cite{agarwal1994fast} to learn XPath-based rules from human annotated sample pages, and ~\cite{anton2005xpath} also  learns XPath-compatible wrappers.
While these techniques can extract HTML elements, they cannot perform finer-grained string processing \emph{inside} HTML elements.
%These systems learn rules that can only extract HTML elements. 
%In contrast, programs learned by our~\toolname system are able to perform more fine-grained extraction of substrings inside an HTML element. 
In contrast, \textsc{FlashExtract}~\cite{flashextract} can perform some text manipulation inside HTML elements\footnote{{We were not able to experimentally compare against {\sc FlashExtract} because their released implementation in Prose does not support text manipulation in HTML elements.}}; however, unlike our approach, it does not use neural constructs, making it difficult to apply this technique to structurally heterogeneous websites.
Recent work~\cite{iyer2019synthesis} targets data extraction from heterogeneous sources by combining ideas from program synthesis and machine learning. However, this approach requires significant number of \emph{manually} labeled samples since it relies on first training an ML model. In contrast, our technique uses pre-trained models and a small amount of training data.

Recent work by \citet{raza2020web} proposes {\sc HYB}, a synthesis-driven web data extraction technique that is now deployed in the Microsoft Power BI product.
This technique is also based on program synthesis and uses a combination of top-down and bottom-up search. As shown in our evaluation, \toolname performs significantly better than their approach; we believe this is due to the fact that our method is based on a neurosymbolic DSL. 

There is also a line of work~\cite{chasins2018rousillon, barman2016ringer, chasins2015browser, chasins2017skip} for learning web automation macros using a programming-by-demonstration approach. These techniques perform scraper synthesis by recording user interactions with a few webpages and then generalize these interactions into a programmatic webpage scraper. In contrast to our approach, these techniques target structurally similar pages (e.g., different Amazon products) and use a different type of input, namely demonstrations.



%While this technique does not require much supervision from humans, it performs worse than our tool on heterogeneous web pages as shown in our evaluation. In particular, our tool is able to perform better due to the use of a novel neuro-symbolic DSL as well as the combination of program synthesis and ML techniques. 



 %Furthermore, our technique combines optimal synthesis and self-supervision, as opposed to using a pure inductive program synthesis approach.  
 %In contrast, our technique is based on PBE and uses a neuro-symbolic DSL. 



% \begin{itemize}
%     \item Wrapper induction (DB-work) \xinyu{not sure what this isx}
%     \item Web-scale information extraction with vertex \xinyu{cited  paper}
%     \item FlashExtract \xinyu{cited} 
%     \item Sarah Chasins stuff \xinyu{cited} 
%     \item SIGMOD paper from Sumit 2020 \xinyu{cited}
% \end{itemize}


\paragraph{Information extraction from text} Much of the IE literature (e.g., relation extraction  \cite{mintz09distant}) is confined to a given database schema. Among IE frameworks,   ``slot-filling'' approaches   \cite{freitag00,patwardhan2007} typically require at least medium-sized training sets to work on  specific schemas, %There is no ``free lunch'': 
and most few-shot approaches \cite{HanEtAl2018,SoaresEtAl2019} use a pre-trained model and perform further training on text that expresses the desired relations in a similar fashion to the target domain.
In contrast, open information extraction techniques\cite{etzioni08openie} aim to retrieve data in an ontology-free way that can theoretically be used for downstream tasks like question answering \cite{choi15scalable}. However, this information is extracted primarily from textual relations rather than structured formatting; even graph-based approaches use graphs over textual relations only \cite{qian19graphie}. Therefore, these approaches do not work well in settings (such as ours) that 
involve a combination of tree structure and free-form text. 
%here a combination of text structure and DOM structure are necessary to address the task.

\paragraph{Information extraction from semi-structured data} Recent work has begun to tackle the problem of semi-structured data, particularly interactions between tables and natural language. Prior work looks at extracting lists from the web \cite{liang2014}, answering questions from tables \cite{pasupat15wikitableq}, verifying facts from tables \cite{chen19tabfact}, or generally extracting information from tables \cite{wu18fonduer}. However, much of this work assumes access to large training sets or relies heavily on the structure of tables.
%so it is not applicable to our more flexible extraction setting.

Two recent efforts have tackled the problem of IE from semi-structured data in a setting similar to ours \cite{lockard20zeroshotceres,lin20freedom}. However, to use these techniques in our setting, we would have to first run their tools
%\footnote{Code is not available for either paper.} 
to extract a knowledge base, and then interpret our questions into some kind of semantic representation that we can execute against the extracted knowledge base. In contrast to such an approach, our work instead \emph{dynamically} learns the relation to extract from the question, specified keywords, and examples. %meaning that it has additional supervision. 

\begin{comment}


\xinyu{Recent work~\cite{iyer2019synthesis} also combines ideas from program synthesis and machine learning for information extraction from heterogeneous semi-structured data (such as web pages and machine-generated emails). 
In particular, it first runs a machine learning model to obtain an initial extraction, which is then fed into a program synthesizer as the specification. This synthesizer produces a set of programs that covers the initial extraction. Then, it runs these programs to obtain a second extraction, which is used to re-train the machine learning model. The re-training and re-synthesizing process is applied iteratively to obtain a final high-quality extraction. 
In comparison, our technique uses a neuro-symbolic DSL that tightly combines machine learning models and symbolic programs, rather than having two separate languages. Our technique then uses a symbolic technique to find all optimal neuro-symbolic programs given training samples and applies machine learning to select the most generalizable program. 
}
\end{comment}


\paragraph{Question answering} Beyond the table-based question answering approaches listed above, there is little work on question answering over text that can be directly applied to our setting. BERT-based \cite{bert} models applied to datasets such as SQuAD \cite{squad} only work well on input that is completely unstructured text. While there are some recent efforts on question answering with more programmatic structures \cite{gupta20neural} for tasks like DROP \cite{dua19drop}, these systems are highly specialized to applications like answering numerical questions.
%and do not have the broad capabilities needed for our task.

\paragraph{Quantitative program synthesis}
There has also been recent work on optimal program synthesis with respect to a quantitative objective. 
For example,~\citet{metasketch} introduce a general framework for optimal program synthesis where the search space is represented by a set of sketches. Their technique uses the objective function together with a gradient function to direct the search. In contrast to~\citet{metasketch}, our work specifically targets the web question answering domain, uses a neurosymbolic DSL, and employs an objective function that is based on program semantics. While ~\citet{metasketch}, in principle, also support semantic objective functions, they require the objective function to be reducible to a decidable theory, which  does not hold in our case due to the use of neural primitives.
\textsc{QuaSi}~\cite{hu2018syntax} also considers the problem of synthesis with quantitative objectives, but it requires the objectives to be syntactic. 
Other existing synthesis techniques~\cite{flashfill, wang2017program, wang2017synthesis},  are mostly \emph{qualitative}, although they implicitly use a ranking function as an inductive bias to help with generalization. However, such ranking functions are quite restricted and  mostly syntactic (e.g., based on program size).


\paragraph{Neurosymbolic DSLs.}

There has been recent interest in neurosymbolic DSLs that include both logical and neural components. For instance, neural module networks~\cite{andreas2016neural,andreas2016learning} dynamically compose DNNs for tasks like predicting object attributes in images~\cite{mao2019neuro} or identifying numbers  in text~\cite{gupta20neural}. However, these techniques use purely neural components (even for operations like  filtering and counting), which significantly increases sample complexity. Recent approaches have trained combinations of neural and logical components  by backpropagating through such programs~\cite{gaunt2017differentiable,valkov2018houdini,shah2020learning}. There has also been work on synthesizing neurosymbolic programs to represent structure in images~\cite{ellis2018learning,young2019learning} and reinforcement learning policies~\cite{inala2020learning,anderson2020neurosymbolic}. Overall, existing approaches largely focus on simultaneously learning the program structure and the DNN parameters. Hence, they are limited to very simple programs and neural components, as they need to optimize  neural network parameters using backpropagation. In contrast, our work is designed to incorporate state-of-the-art DNNs such as BERT, which take significant time to train. In addition, we search over tens of thousands of programs by relying on pretrained DNN models and by developing novel deduction techniques for optimal synthesis.

\paragraph{Multi-modal program synthesis.} There has been growing interest in program synthesis from multiple modalities of specifications. For instance, several works have used a combination  of natural language  and input-output examples to synthesize regular expressions, data wrangling and string manipulation programs,  SQL queries, and temporal logic formulas \cite{regel, mars, raza2015, duoquest, gavraninteractive}. Our technique can also be viewed as an instance of multi-modal synthesis that is based on a neurosymbolic programming language.


% \paragraph{ML for synthesis?}


==> WebExtract arxiv/self-supervision.tex <==
\section{Program Selection via Transductive Learning}~\label{sec:self-supervision}



Our optimal synthesis algorithm outputs all programs that have optimal $F_1$ score on the labeled training data. However, 
not all of these programs generalize well to new inputs. 
In this section, we present a technique based on transductive learning \cite{zhu05survey} that selects a program that generalizes well beyond the training examples. 
%\xinyu{suggesting a rewrite above. my main problem with previous sentence is it does not flow quite well: why do we have to select a single program only because these programs do not generalize equally well? for example, we can use other approaches to get outputs for the test data instead of selecting a program. we are just proposing an approach based on selecting a program but this is not the only solution.}
%these programs may not generalize equally well to new inputs. Thus, we need to select a single program that generalizes well beyond the training examples.

We describe our algorithm (summarized in Figure~\ref{alg:selects}) for selecting a program that generalizes well to the test set. At a high level, our selection method must satisfy two objectives. First, it should select a program that generalizes well in terms of $F_1$ score. Empirically, we observe that a large fraction of optimal programs achieve  good $F_1$ score on the test set, so a randomly chosen program has good $F_1$ score on average. However, we also want to minimize variance---in many cases, a sizable fraction of programs perform quite poorly, so a randomly chosen program may have  poor $F_1$ score. Our selection method is designed to select a good program while avoiding these poorly performing programs.

%\greg{[I don't know whether this is good]
%[idk how to really justify this}
The key concept underlying our approach is to use an \emph{ensemble} of the optimal programs $\Pi^*$ generated by our synthesis algorithm; that is, we aggregate predictions over a large random sample of optimal programs. Such an ensemble would address both of the above points. Ensembles of multiple models typically generalize better than the individual models since the errors made by individual models tend to average out~\cite{opitz1999popular}. For the same reason, they also tend to reduce the variance in performance~\cite{dietterich2000ensemble}. However, directly using an ensemble instead of an individual program has a few drawbacks. First,  an ensemble is significantly less interpretable than an individual model. Second, since an ensemble includes many programs, there is a large computational cost to using the ensemble  if the learned model is to be used over and over again.
%: an individual program learned on a few examples may exhibit bad behavior in some cases, but an ensemble of many such imperfect programs will have less varied behavior.

%

\begin{figure}[t]
\vspace{-10pt}
\small
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{Select}{$\examples, \inputexamples, \Pi^*$}
\Statex\Input{training examples $\examples$, unlabeled input examples $\inputexamples$, optimal programs $\Pi^*$.}
\Statex\Output{optimal program $\pi^*$ on the transductive learning objective.}
\State draw i.i.d. samples $\pi_1,...,\pi_{\mathcal{N}}\sim\Pi^*$;
\State construct ensemble $\Pi_E=\{\pi_1,...,\pi_{\mathcal{N}}\}$;
\State compute the output $\outputexamples_j\in\Pi_E$ for $\pi_j$ according to Eq.~\ref{eqn:ensembleoutputs};
\State compute $L(\pi)=\sum_{j=1}^{\mathcal{N}}L(\pi;\inputexamples,\outputexamples_j)$ for each $\pi\in\Pi_E$;
\State \Return $\pi^*=\operatorname*{\arg\max}_{\pi\in\Pi_E}L(\pi)$;
\EndProcedure
\end{algorithmic}
\end{algorithm}
\vspace{-35pt}
\caption{Program Selection Algorithm.}
\label{alg:selects}
\end{figure}

Thus, our algorithm first builds the ensemble and then \emph{compresses} it into a single program by leveraging  the \emph{unlabeled} training data. In particular, it constructs an ensemble $\Pi_E$ by sampling $\mathcal{N}$ optimal programs returned by the synthesis algorithm (lines 2--3). Then, it uses the ensemble to generate soft labels for the unlabeled webpages and returns the program $\pi^*$ that minimizes loss $L(\pi^*)$ with respect to these soft labels. We describe our approach in more detail below. For conciseness, we give a high-level sketch of our derivations, and provide details in the Appendix.

%Unlabeled data is much easier to obtain than labeled data.
%Then, our algorithm uses \emph{self-supervised learning} for program selection. At a high level, it uses the ensemble to generate plausible outputs $o\in\outputexamples$ for the unlabeled input examples $i\in\inputexamples$. Then, it returns the best program in $\pi^*\in\Pi^*$ according to these self-generated labeled examples $(\inputexamples,\outputexamples)$.
%Finally, for computational tractability, rather than using the entire set $\Pi^*$, our algorithm uses an \emph{ensemble} $\Pi_E$ of i.i.d. samples from $\Pi^*$.
%Essentially, the unlabeled data allows us to distill this ensemble down into a single program which performs similarly to the ensemble on the unlabeled data but which is more tractable to run at test time.
%We describe these components in detail below.

%%%%%%%%%%%%%%%%
% OLD STATISTICAL ASSUMPTIONS
%\paragraph{\red{Statistical Assumption}} \red{ In the remainder of this section, we assume a standard probabilistic model based on the semi-supervised learning literature~\cite{semisuperviseassump}. That is, we have:
%\small
%\begin{align}
%\label{eqn:selfsupervisedassump}
%    p(\inputexamples, \outputexamples, \examples, \pi) = p(\outputexamples \mid \inputexamples, \pi) \cdot p(\inputexamples) \cdot p(\examples \mid \pi) \cdot p(\pi)
%\end{align}
%\normalsize
%In other words,  the outputs ($\outputexamples$) only depend on the unlabeled inputs ($\inputexamples$) and the program ($\pi$).
%}

\paragraph{Transductive learning objective.}
Given (i) labeled examples $\examples$, (ii) unlabeled inputs $\inputexamples$, and (iii) optimal programs $\Pi^*$ returned by  {\sc Synthesize}, our algorithm finds a program $\pi \in \Pi^*$ that minimizes the following objective:
\begin{align}
\label{eqn:selfsupervisedobj}
\tilde{L}(\pi;\examples,\inputexamples)=\mathbb{E}_{p(\outputexamples\mid\inputexamples,\examples)}[L(\pi;\inputexamples,\outputexamples)].
\end{align}
The expression $L(\pi;\inputexamples,\outputexamples)$ is a loss function we wish to minimize in a standard supervised learning fashion using $(\inputexamples, \outputexamples)$ as the training dataset---e.g., we could take it to be the negative $F_1$ score. However, the difficulty is that we do not know the labels $\outputexamples$ for the inputs $\inputexamples$. Thus, we take the expectation with respect to a distribution $p(\outputexamples\mid\inputexamples,\examples)$ that leverages information from the labeled examples. As described in detail below, this distribution is constructed by using an ensemble of programs synthesized based on $\examples$ to assign soft ``pseudo-labels'' to $\inputexamples$.

%, but we can compute an expectation with respect to the label distribution $p(\outputexamples\mid\inputexamples,\examples)$ from the ensemble, giving us a soft pseudo-label.


\paragraph{{Generating} labels via program ensembling.}

Next, we describe how to construct the distribution $p(\outputexamples\mid\inputexamples,\examples)$. We do this in two steps: first, by defining a distribution $p(\pi' \mid \examples)$ over (optimal) programs conditioned on the input data, then using the fact that these programs are deterministic to compute $p(\outputexamples \mid \pi', \inputexamples)$.
%\todo{greg rearranged this section}

We define our distribution $p(\pi'\mid\examples)$ to assign probability mass \emph{only} to programs in $\Pi^*$, those that best satisfy the given examples $\examples$.\footnote{We note that other choices are possible (e.g., prioritizing smaller programs, including some probability on erroneous programs, etc.); we found this choice to work well empirically.}
%\footnote{There are other possibilities here, such as defining a distribution that places a small amount of probability mass over erroneous programs as well. However, with such a large number of optimal programs given that the examples do not fully specify the task, this nevertheless leads to a suitable distribution over outputs.}
Ideally, we could use
%\begin{align*}
%p(\pi\mid\examples)=\frac{\mathbbm{1}(\pi\in\Pi^*)}{|\Pi^*|},
%\end{align*}
the uniform distribution over optimal programs $\Pi^*$. However, a key difficulty is that summing over all programs $\pi\in\Pi^*$ is intractable since the cardinality of $\Pi^*$ is too large in practice. Thus, we instead approximate this distribution by constructing an ensemble $\Pi_E=\{\pi_1,...,\pi_{\mathcal{N}}\}$, where $\pi_i\sim\text{Uniform}(\Pi^*)$ are i.i.d. samples and where $\mathcal{N} \in \mathbb{N}$ is a hyperparameter, and then using
\small
\begin{align}
\label{eqn:selfsuperviseddist}
p(\pi\mid\examples)=\frac{\mathbbm{1}(\pi\in\Pi_E)}{\mathcal{N}}
\end{align}
\normalsize
%\noindent\red{More details of this derivation can be found in the Appendix.}

Finally, given this distribution, we have
\small
\begin{align}
\label{eqn:derivation}
p(\outputexamples\mid\inputexamples,\examples)
&= \sum_{\pi'\in\Pi}p(\pi'\mid\examples)\cdot p(\outputexamples\mid\pi',\inputexamples) \\
&= \sum_{\pi'\in\Pi}p(\pi'\mid\examples)\cdot\prod_{k=1}^K \mathbbm{1}(\outputexamplee_k=\pi'(\inputexamplee_k)) \nonumber
\end{align}
\normalsize
where the second step follows from the fact that our programs are deterministic and each place probability 1 over a single output.
%where $p(\pi'\mid\examples)$ is a distribution over programs $\pi'$ given the labeled training data. 


\paragraph{Program selection.}

Finally, our algorithm aims to select
\small
\begin{align}
\label{eqn:selectedprog}
\pi^*=\operatorname*{\arg\min}_{\pi\in\Pi_E}\tilde{L}(\pi;\examples,\inputexamples).
\end{align}
\normalsize
i.e., the program that minimizes the loss with respect to the ensemble. 
%In principle, we want to search over all programs here, but because this search is intractable, we instead approximate this by searching over the samples drawn to construct our ensemble $\Pi_E$--- i.e., we select
%\begin{align}
%\label{eqn:selectedprog}
%\pi^*=\operatorname*{\arg\min}_{\pi\in\Pi_E}\tilde{L}(\pi;\examples,\inputexamples),
%\end{align}
We now describe how to evaluate $\tilde{L}(\pi;\examples,\inputexamples)$. 

First, we precompute the possible outputs
\small
\begin{align}
\label{eqn:ensembleoutputs}
\outputexamples_j=(\pi_j(\inputexamplee_1),...,\pi_j(\inputexamplee_K))\qquad(\forall\pi_j\in\Pi_E),
\end{align}
\normalsize
in which case we have
\small
\begin{align*}
p(\outputexamples\mid\inputexamples,\examples)
&=\frac{1}{\mathcal{N}}\sum_{\pi'\in\Pi_E}\prod_{k=1}^K\mathbbm{1}(\outputexamplee_k=\pi'(\inputexamplee_k)) \\ &=\frac{1}{\mathcal{N}}\sum_{j=1}^{\mathcal{N}}\mathbbm{1}(\outputexamples=\outputexamples_j).
\end{align*}
\normalsize
In other words, when evaluating $p(\outputexamples\mid\inputexamples,\examples)$, we only need to account for outputs $\outputexamples_j$ according to programs $\pi_j\in\Pi_E$. Thus, we have:
\small
\begin{align}
\tilde{L}(\pi;\examples,\inputexamples)
&=\sum_{\outputexamples}p(\outputexamples\mid\inputexamples,\examples)\cdot L(\pi;\inputexamples,\outputexamples)\\  &=\frac{1}{\mathcal{N}}\sum_{j=1}^{\mathcal{N}}L(\pi;\inputexamples,\outputexamples_j). \label{eqn:derivationgoal}
\end{align}
\normalsize
%Finally, we need to define the probability $p(\pi\mid\inputexamples,\outputexamples)$, which intuitively is the supervised learning objective for input-output examples $(\inputexamples,\outputexamples)$. We assume given a loss function $L(\pi;\inputexamples,\outputexamples)\in\mathbb{R}$ (e.g., the negative $F_1$ score), and use
%\begin{align*}
%p(\pi\mid\inputexamples,\outputexamples)=\frac{1}{Z}\exp(-L(\pi;\inputexamples,\outputexamples)),
%\end{align*}
%where $Z$ is a normalizing constant. Then, we have
%\begin{align*}
%J(\pi;\examples,\inputexamples)
%&=-\frac{1}{N\cdot Z}\sum_{j=1}^NL(\pi;\inputexamples,\outputexamples_j).
%\end{align*}
Substituting into Eq.~\ref{eqn:selectedprog}, our algorithm selects the program
\begin{align}
\label{eqn:selectedprog2}
\pi^*=\operatorname*{\arg\min}_{\pi\in\Pi_E}\sum_{j=1}^{\mathcal{N}}L(\pi;\inputexamples,\outputexamples_j),
\end{align}
which is equivalent to Eq.~\ref{eqn:selectedprog} since $\mathcal{N}$ is a positive constant.


==> WebExtract arxiv/synthesis.tex <==
\section{Optimal Neurosymbolic Synthesis} \label{sec:synthesis}

In this section, we describe our  algorithm for synthesizing  \emph{all} programs that achieve optimal $F_1$ score on a given set of training examples. At a high level, our method is based on enumerative search but employs two ideas that allow it to  scale better: First, we \emph{decompose} the task of synthesizing  extractors from that of synthesizing guards; this decomposition significantly reduces the space of programs we need to consider. Second, we exploit a certain \emph{monotonicity property} of our DSL to prune programs that are guaranteed to be sub-optimal in terms of their $F_1$ score.

%\red{For the sake of clarity, we first formally define an example:}

%\begin{definition}{\bf (\red{Example})} Each example in $\examples$ is a pair $\langle (N, W), Y \rangle$, where $N$ is a set of nodes, $W$ is the input webpage, and $Y$ is a set of extracted texts.
%\end{definition}

%\red{With this definition, we are able to use $N$ to keep track of the set of current extracted nodes with respect to a specific input webpage during synthesis.}

Our top-level synthesis algorithm is presented in Figure~\ref{alg:top-level}. Given a few training examples $\examples$, a question $\question$, and keywords $\keywordss$, {\sc Synthesize} returns a \emph{set} of programs that achieve optimal $F_1$ score on $\examples$. At a high level, the algorithm considers all possible ways of partitioning the training examples and synthesizes optimal programs for each partition.\footnote{Since our technique only requires a small set of labeled examples, considering all partitions of $\examples$ is computationally tractable.} Intuitively, each partition corresponds to a different way of assigning guards to webpages in the training set, and the overall synthesis algorithm chooses a partition that yields  the best $F_1$ score among all partitions.


\begin{figure}[t]
\small
\vspace{-10pt}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{Synthesize}{$\examples, \question, \keywordss$}
\Statex\Input{training examples $\examples$, question $\question$, and keywords $\keywordss$.}
\Statex\Output{all \dsl programs with optimal $F_1$ score.}
\State $\res \assign \bot$; \ $opt \assign 0$;
\ForAll{$\partition \in \textsf{Partitions}(\examples)$}
\State $bs \assign []$;
\ForAll{$\examples_i \in \partition$}
\State $B \assign \textsc{SynthesizeBranch}(\examples_i, \partition \setminus \cup_{j=1}^i  \examples_j, \question, \keywordss)$;
\State $\emph{bs}.append(B )$;
\EndFor
\If{$\textsf{$F_1$}(bs, \examples) > opt$} 
\State $opt = \textsf{$F_1$}(bs, \examples)$;  $\res \assign \{ bs \} $;
\ElsIf{$\textsf{$F_1$}(bs, \examples) = opt$} 
\State$\res \assign \res \cup \{ bs \} $;
\EndIf
\EndFor
\State\Return $\res$;
\EndProcedure
\end{algorithmic}
\end{algorithm}
\vspace{-0.5in}
\caption{Top-level synthesis algorithm.}
\label{alg:top-level}
\vspace{-0.2in}
\end{figure}

In more detail, the {\sc Synthesize} procedure works as follows. It first generates all possible partitions of the training examples, and then, for  each partition $P = [ \examples_1, \ldots, \examples_n ]$, it generates a set of (optimal) programs  of the form:
\[
\psi_1  \to \lambda x. e_1, \ldots ,  \psi_n \to \lambda x. e_n  
\]
such that examples $\examples_i$  satisfy the $i$'th guard $\psi_i$ and the corresponding extractor $e_i$ achieves optimal $F_1$ score for $\examples_i$. We represent the set of optimal programs for partition $P$ as a list $bs = [B_1, \ldots, B_n]$, where each $B_i$ represents an optimal set of programs for the $i$'th branch.




% For a given partition $P = [ \examples_1, \ldots, \examples_n ]$, the algorithm synthesizes optimal \emph{branch programs} $B_i$ for each set of examples $\examples_i$.
%For each set  of examples $\examples_i \in \partition$ in a given partition $\partition$,  
%a partition $P \in \mathsf{Partitions}(\examples)$ and a set of examples $\examples_i \in P$, 
%the algorithm synthesizes a set of \emph{branch programs} $B$ for $\examples_i$. 
In particular, a \emph{branch program} $b \in B_i$ is a pair ($\guard, \stringExt$) consisting of a guard and an extractor, and we represent a set of branch programs as a mapping $B_i$ from guards to a set of extractors $E$. 
% \xinyu{why is it (G, E)? according to fig.5, it's $(\psi, E)$? I wonder if it would make things more clear by making this ``branch program'' more explicit in the grammar (like creating a new symbol for it)?}
Thus,  $B_i$ represents all  branch programs $(\guard, \stringExt)$ satisfying the following three properties:
\begin{enumerate}[leftmargin=*]
    \item The guard $\guard$ evaluates to true for all examples in $\examples_i$. 
   \item The guard $\guard$ evaluates to false for $\examples \backslash (\examples_1 \cup \ldots \cup \examples_i)$.\footnote{{Since a guard is only evaluated if previous guards evaluate to false, we only require $\psi$ to differentiate between the current set of examples and the examples that have not yet been considered.}}
   \item The extractor $\stringExt$ achieves optimal $F_1$ score for examples~$\examples_i$.
\end{enumerate}

%Finally, the return value of {\sc Synthesize} is the set of all optimal programs among all possible ways of partitioning the training examples. 

%The {\sc Synthesize} procedure represents top-level programs in the DSL as a list $bs = [(B_1, $F_1$^1), \ldots, (B_n, $F_1$^n)]$. More formally, $bs$ represents the set of all programs of the form:
%\[
%\psi_1  \to \lambda x. e_1, \ldots ,  \psi_n \to \lambda x. e_n  
%\]
%where $bs[i] = (B_i, \_), \psi_i \in \mathsf{Domain}(B_{i})$ and $e_i \in B_i[\psi_i] $. Finally, the return value of {\sc Synthesize} is a set 


%Thus, the combination of all branch programs for a given partition $P$ corresponds to set of optimal programs for that partition, and the synthesis algorithm returns all programs that maximize the $F_1$ score across all partitions. 

\paragraph{Synthesizing branch programs.} Next, we consider the {\sc SynthesizeBranch} procedure (Figure~\ref{alg:branch}) for generating optimal branch programs for a given set of examples. As mentioned earlier, there are two important ideas underlying this algorithm: First, we decompose the branch synthesis problem into two separate sub-problems (one for synthesizing guards, and one for synthesizing extractors). Second, we prune the search space by inferring an upper bound on the optimal $F_1$ score that can be achieved by partial branch programs. 


In more detail, the {\sc SynthesizeBranch} procedure works as follows. For a given set of positive examples $\examples^+$ and negative examples $\examples^-$, it first synthesizes a guard $\psi$ that separates $\examples^+$ from $\examples^-$ (line 4) and then generates the set of all optimal extractors using $\psi$ (line 8). Note that there may be multiple guards in our DSL that distinguish $\examples^+$ from $\examples^-$. While our algorithm considers all possible guards (loop in lines 3--12), it does so \emph{lazily} --- i.e., it only synthesizes  the next guard after synthesizing optimal extractors for the previous guards. As we will see shortly, such lazy enumeration strategy is useful because it improves the pruning power of the guard synthesis algorithm. 




Now, let us consider each iteration of loop in lines 3--12. First, given a guard $\guard$ separating $\examples^+$ and $\examples^-$ (line 4), our technique infers an \emph{upper bound} on the $F_1$ score of any branch program using $\guard$ as its guard. In particular, we can do this because the extractors in our DSL are monotonic with respect to recall: If extractor $e'$ appears as a sub-expression of $e$, then the recall that can be achieved by extractor $e$ cannot be more than that of $e'$. Furthermore, since the extractor operates over the tree nodes $N$ returned by its corresponding guard, the recall can only decrease  with respect to $N$'s contents.


Our algorithm uses this observation at line 6 of  {\sc SynthesizeBranch}  by using the {\sc UB} function for computing an upper bound on branch programs using guard $\psi$. In particular, let $\nodeExt$ denote the section locator used in guard $\guard$. Then, we can obtain an upper bound for any branch program over $\guard$ using the following formula:
\small
\begin{equation}
\textsf{UB}(\nodeExt, \examples) = \frac{ 2\cdot \mathsf{Recall}(\nodeExt, \examples)}{1+ \mathsf{Recall}(\nodeExt, \examples)} \label{eq:ub}
\end{equation}
\normalsize
where  $\mathsf{Recall}(\nodeExt, \examples)$ for a section locator $\nodeExt$ and examples $\examples$ is defined as follows:
\small
\[
 \frac{\{ t  \ | \ t \in \texttt{\small ExtractContent}(\nodeExt(W)), W \in \examples_{\rm in} \} \cap \{t \ | \  t \in \examples_{\rm out}\} }{\{ t \ | \  t \in \examples_{\rm out}\}}
\]
\normalsize
where $t$ represents a token.

That is, our upper bound computation assumes  maximum possible precision (i.e., $1$) and maximum recall for any extractor using section locator $\nu$. Since $\mathsf{UB}(\nodeExt)$ gives an upper bound on the $F_1$ score of any branch program with guard $\guard$, we do not need to consider extractors for $\guard$ if   $\mathsf{UB}(\nodeExt)$ is less than the maximum $F_1$ score encountered so far (line 6).  


%It iteratively searches through the space of all possible branch programs,

%where each iteration of the loop  in lines 3--12 infers a new classifier (i.e., guard) $\psi$ that evaluates to true for $\examples^+$ and false for $\examples^-$ (line 4). 
%Guard synthesis is done lazily using the {\sc GetNextGuard} procedure (line 4) that we will explain later. 
%Then, given a guard $\guard$ separating $\examples^+$ and $\examples^-$, the algorithm infers an upper bound $b$ on the $F_1$ score of any branch program using $\guard$  and  discards  $\guard$ if $b$ provably less than the optimal $F_1$ score encountered so far. To see how to obtain such an upper bound, let $\nodeExt$ be the section locator used in guard $\guard$. Now, recall that any extractor starts from the nodes $N$ computed by section locator $\nodeExt$ and \emph{refines} the content of those nodes using the {\tt Filter}, {\tt Substring}, and {\tt Split} operations. Thus, if the content of nodes $N$ achieves a \emph{recall} of $r$, then any extractor obtained from $N$ will \emph{only decrease} $r$. Thus, we can use this idea to compute an upper bound on the $F_1$ score of any branch extractor using $\guard$ as follows:

% \[
% \textsf{UB}(\nodeExt, \examples) = \frac{ 2\cdot \mathsf{Recall}(\nodeExt, \examples)}{1+ \mathsf{Recall}(\nodeExt, \examples)}
% \]
% where $\nodeExt$ denotes the section locator used in guard $\guard$, and  $\mathsf{Recall}(\nodeExt, \examples)$ for a section locator $\nodeExt$ and examples $\examples$ is defined as follows:
% \[
% \frac{\{ s  \ | \ s \in \texttt{\small ExtractContent}(\nodeExt(W)), W \in \examples_{\rm in} \} \cap \{s \ | \  s \in \examples_{\rm out}\} }{\{s \ | \  s \in \examples_{\rm out}\}}
% \]
% In other words, the procedure \textsf{UB} used at line 6 computes an upper bound on $F_1$ score by assuming  maximum possible precision (i.e., $1$) and maximum recall for any extractor using section locator $\nu$. Since $\mathsf{UB}(\guard.\nodeExt)$ gives an upper bound on the $F_1$ score of any branch program with guard $\guard$, we do not need to consider extractors for $\guard$ if   $\mathsf{UB}(\guard.\nodeExt)$ is less than the maximum $F_1$ score encountered so far (line 6). 

Assuming $\guard$ is not provably sub-optimal, {\sc SynthesizeBranch} proceeds to construct optimal extractors for the synthesized guard $\guard$ (lines 7--12). To  decompose extractor synthesis from guard inference, we first compute separate input-output examples for the extractor by calling  \textsf{PropagateExamples} at line 7. In particular, this procedure executes the synthesized section locator $\nodeExt$ on the input webpages to obtain new input-output examples $\examples'$ for the extractor and invokes  {\sc SynthesizeExtractors}  on $\examples'$. % to obtain extractors that yield optimal $F_1$ score on $\examples'$.
Finally, if the branch programs associated with guard $\guard$ improve upon (or yield the same) $F_1$ score, the result set $R$ is updated.\footnote{Since branches that use guards with the same section locator have the same set of optimal extractors, the calls to {\sc SynthesizeExtractors} can be memoized across different iterations within the {\sc SynthesizeBranch} procedure. We omit this to simplify presentation.}

\begin{figure}[t]
\small
\vspace{-10pt}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{SynthesizeBranch}{$\examples^+, \examples^-, \question, \keywordss$}
\Statex\Input{Pos/neg examples $\examples^+, \examples^-$; question $\question$;  keywords $\keywordss$}
\Statex\Output{Branch programs represented as a mapping $R$ from guards to extractors  such that for each $(\psi, E) \in R$ (1) $\psi$ classifies $\examples^+, \examples^-$ and (2) $E$ achieves maximum $F_1$ score for $\examples^+$.}
\vspace{0.05in}
\State $\res \assign \bot$; $opt \assign 0$;
\While{$\text{true}$}
\State $\guard \assign \textsc{GetNextGuard}(\examples^+, \examples^-, Q, K, opt)$;
\If{$\guard = \bot$} \textbf{break};
\EndIf
%\State $ns \assign \textsf{GetNodeExtractor}(\guard)$;
\If{$\textsf{UB}(\guard.\nodeExt, \examples^+) < opt $} \textbf{continue}; 
\EndIf
\State $\examples' \assign \textsf{PropogateExamples}(\examples^+, \guard, Q, K)$;
\State $(E, F_1) \assign \textsc{SynthesizeExtractors}(\examples',  Q, K, opt)$;
\If{$F_1 > opt$} 
\State $opt \assign F_1$;  \ $\res \assign \{ (\guard, E)  \}$;
\ElsIf{$F_1 = opt$} 
\State $R[\psi] \gets E$
\EndIf
\EndWhile
\State \Return \res
\EndProcedure
\end{algorithmic}
\end{algorithm}
\vspace{-0.4in}
\caption{Algorithm for synthesizing branch programs.}
\label{alg:branch}
\end{figure}

\paragraph{Extractor synthesis.} Next, we describe the {\sc SynthesizeExtractors} procedure (Figure~\ref{alg:extractor}) for finding extractors with optimal $F_1$ score for a given set of input-output examples.  This procedure uses \emph{bottom-up} enumeration with pruning based on $F_1$ scores to reduce the search space. In particular, we use bottom-up rather than top-down enumeration because doing so allows us to  more easily exploit the monotonicity property of the DSL with respect to recall. 


% because pruning based on $F_1$ scores relies on first obtaining the results of the subprogram executed on the examples.
% In particular, we use bottom-up rather than top-down enumeration because pruning based on $F_1$ scores is only possible if we use this bottom-up strategy.

In more detail, {\sc SynthesizeExtractors} maintains a worklist $\worklist$ of complete extractors; and, in each iteration, it dequeues one extractor and expands it by applying all possible grammar productions for {\tt Substring}, {\tt Filter}, and {\tt Split} (line 8). A new extractor $\stringExt'$ is  added to the worklist only if $\textsc{UB}(\stringExt', \examples)$ (i.e., $F_1$ score upper bound for $\stringExt'$) is greater than or equal to the previous upper bound $s_o$ (line 9). As described earlier, we compute an upper bound on extractors generated from $e'$ by using $1$ for precision and the recall of $e'$ on the given set of examples. As before, this pruning strategy exploits the fact that if $e_1$ is a subprogram of $e_2$, then $\mathsf{Recall}(e_1, \examples) \geq \mathsf{Recall}(e_2, \examples)$ for any set of examples $\examples$. 

\begin{figure}
\small
\vspace{-10pt}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{SynthesizeExtractors}{$\examples,  \question, \keywordss, opt$}
\Statex\Input{Examples $\examples; $question $\question$;  keywords $\keywordss$}
\Statex\Input{Lower bound $opt$ on $F_1$}
\Statex\Output{Extractors $E_o$ with optimal $F_1$ score $\fonescore_{o}$ on $\examples$.}
\State $E_{o} \assign \emptyset$; \ $\fonescore_{o} \assign opt$;
\State $\worklist \assign \{ \texttt{ExtractContent}(x) \}$;
\While{$\worklist \neq \emptyset$}
\State $\stringExt \assign \worklist.remove()$; \ $\fonescore \assign \textsf{$F_1$}(\stringExt, \examples)$;
\If{$\fonescore > \fonescore_{o}$}
$E_{o} \assign \{ \stringExt \}$; $\fonescore_{o} \assign \fonescore$;
\ElsIf{$\fonescore = \fonescore_{o}$} $E_{o}.add(\stringExt)$;
\EndIf
\ForAll{$\stringExt' \in \textsf{ApplyProduction}(\stringExt)$}
\If{$\textsc{UB}(\stringExt', \examples) \geq \fonescore_{o}$}
$\worklist.add(\stringExt')$;
\EndIf
\EndFor
\EndWhile
\State\Return $(E_{o}, \fonescore_{o})$;
\EndProcedure
\end{algorithmic}
\end{algorithm}
\vspace{-30pt}
\caption{Optimal extractor synthesis.}
\label{alg:extractor}
\vspace{-0.1in}
\end{figure}


\paragraph{Lazy synthesis of guards.} The final missing piece of our synthesis algorithm is the {\sc GetNextGuard} procedure (Figure~\ref{alg:guard}) for lazy guard synthesis. In particular, this algorithm is \emph{lazy} in the sense that it yields a single guard at a time rather than returning the set of all guards separating $\examples^+$ from $\examples^-$. Since the guard synthesis algorithm also prunes its search space by computing an upper bound on $F_1$ scores, this lazy enumeration strategy improves  pruning power as the optimal $F_1$ score improves over time. However, despite the lazy nature of the guard synthesis algorithm, our technique is still guaranteed to return all optimal programs.


The guard synthesis algorithm (Figure~\ref{alg:guard})  is  similar to {\sc SynthesizeExtractors} and also performs bottom-up search with pruning. In particular, it maintains a worklist $\worklist$ of section locators. In each iteration, it dequeues one of the section locators $\nodeExt$ and generates all possible guards using $\nodeExt$ (up to some bound). If any of the resulting guards $\guard$ is a classifier between $\examples^+$ and $\examples^-$, then it is returned as the next viable guard.  Once the algorithm enumerates all possible classifiers using the section locator $\nodeExt$, it then generates all possible section locators derived from $\nodeExt$ by using the productions {\tt GetChildren} and {\tt GetDescendants} (lines 7-8). As in the previous algorithms, {\sc GetNextGuard} also computes an upper bound on  $F_1$ score  and adds a new section locator $\nodeExt'$ to the worklist if ${\sf UB}(\nodeExt', \examples^+)$ is no worse than the previous optimal $F_1$ score~$opt$ (line 8).


\begin{theorem}
Let $\examples, Q, \keywordss$ be inputs to the {\sc Synthesize} procedure and let  $p$ be a \dsl  program. Then, the set of programs returned by {\sc Synthesize}($\examples, Q, \keywordss$) includes $p$ if and only if, for any other  \dsl program $p'$,   $F_1(p)  \geq F_1(p')$. 
\end{theorem}
\label{thm:1} 


\begin{figure}
\vspace{-0.15in}
\small
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{GetNextGuard}{$\examples^+, \examples^-, \question, \keywordss, opt$}
\Statex\Input{Pos/neg examples $\examples^+,\examples^-$}
\Statex\Input{Question $\question$; keywords $\keywordss$;  lower bound $opt$ on $F_1$ score}
\Statex\Output{Next guard that classifies $\examples^+$ and $\examples^-$.}
\vspace{0.05in}
\State $\worklist \assign \{ \texttt{GetRoot}(\webpage) \}$;
\While{$\worklist \neq \emptyset$}
\State $\nodeExt \assign \worklist.remove()$;
\ForAll{$\guard \in \textsf{GenGuards}(\nodeExt)$}
\If{$\forall \examplee_{in} \in \examples^+. \semantics{\guard(\examplee_{in},\question,\keywordss)}$ 
$\wedge$
\Statex \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $\forall \examplee_{in} \in \examples^-. \neg \semantics{\guard(\examplee_{in},\question,\keywordss)}$} \textbf{yield} $\guard$;
\EndIf
\EndFor
\ForAll{$\nodeExt' \in \textsf{ApplyProduction}(\nodeExt)$}
\If{$\textsf{UB}(\nodeExt', \examples^+) \geq opt$}
$\worklist.add(\nodeExt')$;
\EndIf
\EndFor
\EndWhile
\State \Return $\bot$;
\EndProcedure
\end{algorithmic}
\end{algorithm}
\vspace{-30pt}
\caption{Lazy enumeration of guards.}
\label{alg:guard}
\vspace{-0.15in}
\end{figure}





\begin{comment}

============= old 


\begin{figure}
\small
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{Synthesize}{$\examples, \question, \keywordss$}
\Statex\Input{Training examples $\examples$, a question $\question$, keyword(s) $\keywordss$}
\Statex\Output{Set of programs $\res$ that achieve optimal $F_1$ score on training examples}
\vspace{0.05in}
\State $\res \assign \varnothing$; \ $\bestf \assign 0$;

\ForAll{$\partition \in \textnormal{\textsf{Partitions}}(\examples)$}
\ForAll{$\examples_i \in \partition$}
\State $\guards_i \assign \mathsf{SynthesizeGuards}(\examples_i, \examples \backslash \{ \examples_1, \ldots, \examples_i\})$
\ForAll{$ns_{ij} \in \textsf{NodeExtractors}(\guards_i)$}
\State $\examples_i' \assign \textsf{PropagateExamples}(ns_{ij}, \examples)$
\State $\extractors_i \assign \mathsf{SynthesizeExtractors}(\examples'_i)$
\EndFor

\EndFor
\State $e_1, \dots, e_{|\partition|} \assign \textsc{SynthesizeExtractors}(\partition)$;
\State $\guard_1, \dots, \guard_{|\partition|} \assign \textsc{SynthesizeGuards}(\partition)$;
\State $p \assign \lambda \question.\keywordss.\webpage \{ \guard_1 \rightarrow e_1, \dots, \guard_{|\partition|} \rightarrow e_{|\partition|} \}$;
\If{$\textsf{$F_1$}(p, \examples) > \textsf{$F_1$}(p_{best}, \examples)$} 
$p_{best} \assign p$;
\EndIf
\EndFor
\State \Return $p_{best}$;
\EndProcedure
\end{algorithmic}
\end{algorithm}
\label{alg:top-level}
\caption{Synthesis algorithm.}
\end{figure}


\begin{figure}
\small
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{Synthesize}{$\examples, \question, \keywordss$}
\Statex\Input{d}
\Statex\Output{d}
\State $p_{best} \assign \bot$;
\ForAll{$\partition \in \textnormal{\textsf{Partition}}(\examples_{in})$}
\State $e_1, \dots, e_{|\partition|} \assign \textsc{SynthesizeExtractors}(\partition)$;
\State $\guard_1, \dots, \guard_{|\partition|} \assign \textsc{SynthesizeGuards}(\partition)$;
\State $p \assign \lambda \question.\keywordss.\webpage \{ \guard_1 \rightarrow e_1, \dots, \guard_{|\partition|} \rightarrow e_{|\partition|} \}$;
\If{$\textsf{$F_1$}(p, \examples) > \textsf{$F_1$}(p_{best}, \examples)$} 
$p_{best} \assign p$;
\EndIf
\EndFor
\State \Return $p_{best}$;
\EndProcedure
\end{algorithmic}
\end{algorithm}
\label{alg:top-level}
\caption{Synthesis algorithm.}
\end{figure}





\begin{figure}
\small
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{SynthesizeExtractor}{$\examples$}
\Statex\Input{d}
\Statex\Output{d}
\State $p_{best} \assign \bot$;
\State $\worklist \assign 
\{ \texttt{GetNodesByKeyword}(\webpage, \keywordss, k, t) \ | \ k \in \mathcal{K}, t \in \mathcal{T}  \}$
\Statex $\ \ \ \ \ \ \ \ \ \ \ \ \ \cup \{ \texttt{GetNodesByQuestion}(\webpage, \question, k) \ | \ k \in \mathcal{K} \}$
\Statex $\ \ \ \ \ \ \ \ \ \ \ \ \ \cup \{  \texttt{GetRoot}(\webpage)  \}$; 
\While{$\worklist \neq \emptyset$}
\State $p \assign \worklist.remove()$;
\State $ub \assign \textsc{UpperBound$F_1$}(p, \examples)$;
\If{$ub \leq \textsf{$F_1$}(p_{best})$} \textbf{continue};
\State $\worklist' \assign \textsc{ApplyProductions}(p)$;
\State $\worklist \assign \worklist \cup \worklist'$;
\ForAll{$p' \in \worklist'$}
\If{$\textsf{$F_1$}(p') > \textsf{$F_1$}(p_{best})$} $p_{best} \assign p'$;
\EndIf
\EndFor
\EndIf
\EndWhile
\State\Return{$p_{best}$;}
\EndProcedure
\end{algorithmic}
\end{algorithm}
\caption{Let's see if you like this.}
\end{figure}



\begin{figure}
\small
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{SynthesizeGuards}{$\examples$}
\Statex\Input{d}
\Statex\Output{d}
\EndProcedure
\end{algorithmic}
\end{algorithm}
\caption{Do we need to write this?}
\end{figure}



\begin{figure*}
\small 
\[
\begin{array}{cr}
\begin{array}{c}
\irule{
\text{p is ns} \ \ S \assign \{ \texttt{GetChildren}(p), \texttt{GetLeaves}(p), \texttt{GetStructured}(p), \texttt{ExtractContent}(p) \}
}{
\vdash p \leadsto S
}
\end{array}
\\ \\ 
\begin{array}{c}
\irule{
\text{p is e} \ \ S \assign \{ \}
}{
\vdash p \leadsto S
}
\end{array}
\end{array}
\]
\caption{Inference rules for \textsc{ApplyProductions}. TBD but this is pretty obvious, do we need to write this?}
\end{figure*}


\end{comment}



